On the state of reporting in crowdsourcing experiments and a checklist to aid current practices

Crowdsourcing is being increasingly adopted as a platform to run studies with human subjects. Running a crowdsourcing experiment involves several choices and strategies to successfully port an experimental design into an otherwise uncontrolled research environment, e.g., sampling crowd workers, mapping experimental conditions to micro-tasks, or ensure quality contributions. While several guidelines inform researchers in these choices, guidance of how and what to report from crowdsourcing experiments has been largely overlooked. If under-reported, implementation choices constitute variability sources that can affect the experiment's reproducibility and prevent a fair assessment of research outcomes. In this paper, we examine the current state of reporting of crowdsourcing experiments and offer guidance to address associated reporting issues. We start by identifying sensible implementation choices, relying on existing literature and interviews with experts, to then extensively analyze the reporting of 171 crowdsourcing experiments. Informed by this process, we propose a checklist for reporting crowdsourcing experiments.

==> CSCW 2021 - Reporting crowd experiments/Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> CSCW 2021 - Reporting crowd experiments/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> CSCW 2021 - Reporting crowd experiments/preamble.tex <==
\section{Preamble}

\textbf{Scope.} This paper aims to propose a datasheet for reporting crowdsourcing experiments. By crowdsourcing experiments, we mean studies that answer research questions/hypotheses using an experimental design (randomized or quasi-experimental) and crowd workers as participants (recruited from a crowdsourcing platform)\footnote{Human subjects should come from an online platform dedicated explicitly to crowdsourcing (paid or volunteering). Further details related to the scope can be found at \url{https://docs.google.com/document/d/1J-0ELGilVNfK_Y6rwX9JLNMupA_apo83FZLE76qz64A/edit?usp=sharing}}.
%
The motivation behind this work is that, currently, there are no standardized guidelines for reporting crowdsourcing projects, and crowdsourcing involves articulating many pieces that can certainly play a role in the results obtained (emphasizing the need for proper reporting).


\textbf{Progress so far.} We have built an initial taxonomy of relevant attributes characterizing crowdsourcing experiments. This taxonomy was derived from different sources 1) guidelines for experimental research, 2) guidelines for crowdsourcing experiments, 3) task design features in crowdsourcing platforms, and 4) papers reporting crowdsourcing experiments. 

We also collected papers by querying on Scopus and checking past HCOMP proceedings. We identified 175 relevant articles from the initial list of 994 documents that we obtained. These relevant studies report crowdsourcing experiments, based on the definition we introduced previously. Using a sample of the relevant papers, we plan to analyze and state of reporting according to the datasheet that we propose in this work.


\textbf{Validity of our work}. To validate our work, we seek to involve experts from the community to review our proposed taxonomy to update and improve it accordingly, growing it into a reporting tool.
%
Guided by our taxonomy, we also plan to rely on existing literature to distill how the different configuration of the parameters of crowdsourcing experiments could play a role in the results (e.g., different task interfaces, payments, instructions, demographics).

In our CSCW poster, we already identified what parameters tend to go underreported, so we are working on doing a complementary analysis, based on simulations from an existing crowdsourcing dataset, of how these underreported settings may flip or "dissolve" the results obtained from the controlled crowdsourcing experiments. Concretely, we are currently evaluating the sampling of workers based on demographics and time of the day, and how this could influence the results.
\gd{there seems to be an assumption that it would be good to report as much as possible. On the other hand, making MTurk output files available to the public may not be desirable as they contain worker IDs (see \url{https://blog.humancomputation.com/?p=5177}). Perhaps it could use useful to a para on the trade-offs between underreporting and overreporting.}
\jr{Regarding the sharing of output datasets, we'd make it clearer that by sharing results (e.g., raw judgments), we also ask for proper anonymization since, indeed, and thanks for sharing the link, workers are not anonymous. And yes, it would be great to discuss under- vs. over-reporting and address this with the datasheet.}

\textbf{Follow-up work}. In this paper, we scope the datasheet to crowdsourcing experiments. However, data collection (e.g., labeling for ML) is also a huge use case for crowdsourcing, and we aim to propose a taxonomy for reporting crowdsourced data collection. AAAI is a potential venue for this work.

==> CSCW 2021 - Reporting crowd experiments/sections/background.tex <==
\section{Background \& Motivation}



Crowdsourcing platforms are being widely adopted as an environment to run experiments with human subjects \cite{DBLP:conf/chi/KitturCS08,DBLP:journals/sigkdd/MasonW09,Paolacci2010RunningEO,Crump2013}. 
% 
\hll{Researchers are leveraging crowdsourcing} to test hypotheses, comparing different study methods, designs or populations, as well as to run studies aiming at observing user behavior. 
For example, crowdsourcing is helping researchers evaluate the impact of different interface designs on user performance, comprehension and understanding \cite{steichen2015supporting,dimara2017narratives,ramirez2019}, assess the difference in performance between users with different expertise, background and even mood levels \cite{wu2016novices,hube2019understanding,xu2019revealing}.   
%
These platforms (e.g., Amazon MTurk) give researchers easy access to a large and diverse population of participants, allowing them to scale experiments previously curbed to constrained laboratory settings. 







Researchers need to articulate many elements to successfully map and run an experiment in a crowdsourcing platform, as depicted in Figure \ref{fig:experiment-mapping}. 
%
The relevance of this is rooted in the need of incorporating more control and safeguards in an otherwise uncontrolled environment \cite{DBLP:conf/dagstuhl/GadirajuMNSEAF15}.
%
For example, an experiment testing the quality of two alternative approaches to text summarization would require researchers to define, among others, i) how to implement the two text summarization conditions as micro-tasks in the crowdsourcing platform (e.g., both conditions in the same task or in different tasks), ii) how to sample and allocate crowd workers to have representative, diverse (e.g., in culture, education or mother-tongue) and comparable groups assigned to both experimental conditions,\footnote{
\hl{While a perfect sampling and allocation strategy (of workers to conditions) may represent an ideal scenario detached from reality, we as researchers should ensure a reasonable balance in the underlying population to avoid confounds affecting the experimental outcome.}
} iii) quality control measures to avoid malicious or low-quality contributions from workers, and iv) task design and configuration, including the user interface, training examples, number of text summaries to show to each contributor, and the compensation for their participation. In doing so, researchers also need to ensure that their entire setup meets ethical standards for research with human subjects.



\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/experiment-mapping.pdf}
  \caption{Mapping an experimental design to a crowdsourcing platform involves articulating many elements (none of which have a unique implementation). These elements constitute sources of variability if not properly reported.}
  \Description{Mapping an experimental design to a crowdsourcing platform involves articulating many elements (none of which have a unique implementation). These elements constitute sources of variability if not properly reported.}
  \label{fig:experiment-mapping}
\end{figure}





While guidelines and best practices have emerged to help researchers navigate the implementation choices and inherent challenges of running experiments in a crowdsourcing environment  \cite{DBLP:conf/icwsm/RogstadiusKKSLV11,Mason2012,Chandler2013}, little attention has been paid to how to \textit{report} on crowdsourcing experiments to facilitate assessment and reproducibility of the research.
If not properly reported, the elements mentioned above constitute sources of variability that can introduce confounds affecting the repeatability and reproducibility of the experiments, and preventing a fair assessment of the strength of the empirical evidence provided.






Reproducibility of experiments is essential in science \cite{DBLP:conf/chi/Wacharamanotham20}. The scrutiny of the research methods, by the academic community, and the development of standardized protocols and methods for communicating results are critical in the production of robust and repeatable experiments. Examples of this can be found in evidence-based medicine where systematic reviews follow a strict elaboration protocol \cite{Prisma}, or, more recently, in the machine learning community where authors are encouraged to follow pre-established checklists or datasheets to communicate their models and datasets effectively \cite{bender-friedman-2018-data,Gebru2019,DBLP:conf/fat/MitchellWZBVHSR19,DBLP:journals/ibmrd/ArnoldBHHMMNROP19,MLReproducibilityChecklist}.
%
Efforts in this regard have been branded under the definitions of \textit{repeatability}, \textit{replicability} and  \textit{reproducibility}, to denote attempts at obtaining 
similar results, by the same or different teams and experimental conditions, under acceptable margins of error \cite{plesser2018reproducibility}. Terminology notwithstanding, the importance of reporting experiments in sufficient detail has long been acknowledged as a fundamental aspect of research and of the scientific process.




The reporting of crowdsourcing experiments should be held to the same standards. Studies, under the umbrella of reproducibility and experimental bias, report on multiple aspects that affect the outcome of crowdsourcing experiments. These aspects include task design (e.g., instructions \cite{DBLP:conf/hcomp/WuQ17}, compensation \cite{DBLP:conf/www/HoSSV15}, task interface \cite{DBLP:conf/chi/SampathRI14}, and time \cite{maddalena2016crowdsourcing} among others), external factors such as the workers' environment \cite{DBLP:journals/imwut/GadirajuCGD17}, platforms \cite{Qarout2019PlatformRelatedFI}, and population \cite{DBLP:conf/wsdm/DifallahFI18} --- all of which serve as the foundation for running user studies.
%
In addition to the standard reporting for experimental research, it is paramount to identify and report the critical aspects and all possible knobs that take part in crowdsourcing experiments.
%
In this regard, existing literature has barely grappled with proposing guidelines that aid the reporting of crowdsourcing experiments, with existing guidelines limited to crowdsourced data collection in the social sciences \cite{Porter2020}.







In this paper we aim to fill this gap. 
We do so by identifying salient issues associated with the reporting of crowdsourcing experiments and propose solutions that can help address these issues. 
Specifically, we derive a \textit{taxonomy of attributes} associated with crowdsourcing experiments and turn this into a checklist for reporting. The checklist aims at facilitating the reporting of crowdsourcing experiments so that they can be repeated and so that a reader can assess if the experiment design matches the desired intent. 
The focus in this paper is on the reporting of  \textit{experiments} ran via crowdsourcing, that is,  studies aiming to answer research questions/hypotheses by following an experimental design, mapping the design to a crowdsourcing task and the features of the platform that supports it, and recruiting crowd workers as subjects.
%
%Not all crowdsourcing tasks are experiments (e.g., data labeling tasks are often not framed as experiments) but the challenges in reporting on experiments are likely to be a superset of those or generic crowdsourcing tasks.
%
\hl{This paper therefore excludes qualitative crowdsourcing studies (e.g., surveys) from its scope and, in general, other kinds of tasks that are not experiments (e.g., data labeling tasks are often not framed as experiments). However, the challenges in reporting on experiments are likely to be a superset of those or generic crowdsourcing tasks.}




\textbf{Contributions.} To aid the reporting of crowdsourcing experiments, we first need to understand the main factors that affect repeatability and that enable assessment of the quality of experiments by reviewers. 
We start by deriving the major design decisions of crowdsourcing experiments that play a role in crowdsourcing tasks and, therefore, on an experiment's outcomes.
%
We do so by following an iterative approach \hl{--- where we rely on literature reviews and interviews with experts ---} and derive a taxonomy of relevant attributes characterizing crowdsourcing studies.
%
Using this taxonomy, we analyze the state of reporting in crowdsourcing literature and identify aspects that are frequently communicated and those that tend to go under-reported. We leverage these observations to discuss potential pitfalls and threats to validity of experiments.
%
With feedback from experts, \hl{we then propose a checklist for crowdsourcing experiments to help researchers be more systematic in what they report.}
%researchers towards more transparent reporting.
%at facilitating the job of understanding and replicating crowdsourcing experiments. 
%This checklist seeks to help experimenters describe their setup in a standardized format and readers to understand the used methodology and how it was implemented, serving as a tool that complements existing experimental research guidelines.
This checklist seeks to help experimenters describe their setup in a standardized format and readers to understand the used methodology and how it was implemented, serving as a tool that complements existing experimental research guidelines


% \hl{We stress that the goal of the type of support we explore here is to contribute to more a transparent reporting that can enable a better  assessment of the validity of experiments, as well as to repeatability. }  



% We aim for the checklist to serve as a resource that guides researchers in what they report, helping them be thorough and systematic in communicating the details of their crowdsourcing experiments (i.e., serving as a reminder,  \textit{``when we are very deep into our data analysis part we forget the basic stuff that should be reported''}).}

==> CSCW 2021 - Reporting crowd experiments/sections/discussion.tex <==



\section{Discussion}

% Y.E >= 65%: input dataset, reward strategy, task interface, number of participants, platform
% Y.E >= 70%: reward strategy, number of participants, selected platform.


% Y.E + Y.I >= 70%: experimental design to task mapping, input dataset, allocation to exp condition, execution of exp conditions, reward strategy, task interface, instructions, rejection criteria, number of participants, platform 



\hl{
The current state of reporting in crowdsourcing research still misses providing details beyond basic attributes associated with task design, quality control, requester, and experiment design and outcome.
%
According to our analysis, at least 70\% of papers report the selected platform, how the experimental design maps and executes, reward strategy, task interface, instructions, rejection criteria, and the number of participants. However, if we consider only explicit reporting, this list narrows to reward strategy, the number of participants, and the selected platform.
%
While these attributes are relatively well-covered, either explicitly or implicitly, most tend to be under-reported by at least 50\% of the papers. Among the six dimensions in our taxonomy, the requester --- with attributes covering the ethics of experiments --- was among the least reported by the papers. These issues open the room for potential threats to validity associated with missing details regarding the experimental design and its operationalization.
}




\hl{
Under-reporting poses the interesting question of why the attributes are poorly reported in the first place and how we can overcome this situation.
%
Our analysis and feedback from experts attribute this issue to the limited guidance and awareness on what needs to be reported. 
%
By providing a checklist and depicting where the research community stands in terms of reporting practices, we expect our work to stimulate additional efforts to move the transparency agenda forward.
%
It is clear from our study that improved transparency in reporting is a shared responsibility among the different stakeholders in the crowdsourcing ecosystem.
} 





\hl{
\textbf{\textit{Researchers}} may be asked to agree to a code of conduct or follow guidelines, like our checklist, to improve the current level of reporting. 
As a \textbf{\textit{research community}}, we need to develop guidelines and best practices (e.g., on how we set up and report experiments) to increase transparency, strength, and reproducibility of crowdsourcing experiments. And such guidelines should also emphasize the ethics and fairness behind experiments.
%
In turn, \textbf{\textit{venues}} need to enforce and adopt higher reporting standards, mirroring the initiatives taking place in other communities.
}



















\hl{
\textbf{\textit{Platforms}} can benefit from the insights and design recommendations emerging from our work and address operational barriers to reporting.
%
Platform providers may aim for solutions that are ``experiment-aware'' (e.g., by offering features to treat experiments as first-class citizens).
%
Indeed, platforms can play a major role in both i) helping task requesters to design experiments that are consistent with accepted ethical guidelines (from informed consent to minimum wage) and ii) helping to generate reports that facilitate publication of relevant experiment information to aid reproducibility.
}


\bigskip

\noindent \hll{
\textbf{Limitations.} It is important to note that the assessment of crowdsourcing experiments in this work is limited to what is reported, which might be an incomplete picture of the design and operationalization of the experiments --- but that is what is eventually available to the community to build upon and replicate.
%
% Furthermore, our analysis of the state of reporting may have (inevitably) missed relevant literature, but we did our best to cover as much research landscape as possible by screening 670 papers and doing a full analysis of 171 articles.
While a systematic process was followed to cover as much research landscape as possible, the search can not be considered an exhaustive account of crowdsourcing experiments in the literature. Yet, the 670 conference papers screened and the 171 analyzed in detail provide a representative sample of the current state of affairs.
%
Also, it is worth noting that we did not manage to cover the four stakeholders we mentioned before, as we did not interview people (e.g., managers and crowd workers) from major crowdsourcing platforms. However, the participants we interviewed possess ample experience designing and executing crowdsourcing experiments in these platforms, with research output published in major SIGCHI conferences; they helped provide thoughtful design and operational angles to the attributes in the taxonomy and the final checklist.
}






            



\section{Conclusion}

The takeaway message is that the characteristics of the crowdsourcing environment pose several challenges to the design and execution of experiments, making them subject to more complex sources of bias. 
%
Therefore, it is of paramount importance to encourage further transparency to aim for higher standards of evidence and reproducibility of results. As we observed, however, we still lack in this regard
%
\hll{--- under-reporting leaves} room for potential threats to validity. This invites a reflection on how valid are current crowdsourcing experiments, how reproducible they are, and whether they comply with ethical standards that ensure fair treatment of crowd workers and their data.
% \hl{It is important to note that we limited our assessment to what is reported, which might be an incomplete picture of how the experiments are actually run --- but that is what is eventually available to the community, and as we have seen, it leaves room for potential threats to validity. This invites a reflection on how valid are current crowdsourcing experiments, how reproducible they are, and whether they comply with ethical standards that ensure fair treatment of crowd workers and their data.
% }



This work pushes crowdsourcing research towards standardized reporting of crowdsourcing experiments. Current guidelines focus on effective task design and practical recommendations for running experiments. But these guidelines somewhat overlook advising researchers on what and how to report the details underlying crowdsourcing experiments. 
%
%
This paper introduced a taxonomy of relevant ingredients characterizing crowdsourcing experiments and used this taxonomy to analyze the state of reporting of a sample of articles published in top venues. This process allowed us to identify gaps in current reporting practices. To help address these issues, we leveraged the resulting taxonomy and feedback from experts to propose a checklist for reporting crowdsourcing studies.


Promising future work avenues include evaluating if and how the checklist aid reproducible research, exploring methods to automatically derive crowdsourcing experiment reports from existing crowd platforms, and  developing a system with crowdsourcing experiments as first-class citizens.







==> CSCW 2021 - Reporting crowd experiments/sections/drec.tex <==


\section{A checklist for reporting crowdsourcing experiments} \label{sec:checklist}
The insights from the literature overview, expert interviews and the state or reporting, paint a daunting image for the reporting of crowdsourcing experiments, calling for the development of better guidelines and resources. In this section we take a small step in this direction, and describe the process that led to the development of a reporting checklist for crowdsourcing experiments. \hl{We stress that the goal of the type of support we explore here is to contribute to more a transparent reporting that can enable a better  assessment of the validity of experiments, as well as to repeatability. }  





\input{sections/methods-checklist}


\subsection{Proposed checklist}

% We use the insights from the analysis to point out the need for a datasheet for reporting on the experiments.

% The process we follow can include some of the steps below:
% \begin{itemize}
%     \item we started from the taxonomy, and tried to report on the relevant attributes of existing (crowdsourcing) papers ourselves. This helped us refine the set of attributes as well as shape the description of the attributes. 
%     \item we then took the papers of experts, and put then in the intended reporting format, and got their feedback. With this we got expert feedback on the datasheet, the relevance of the attributes included, and the clarify of the descriptions. We took their papers in an effort to present them experiments they were already familiar with. Feedback from a producer / consumer perspective (?)
    
%     \item (Not sure) A crowdsourcing experiment where we validated the usability of the datasheet, by going to crowd workers, where we cannot assume specific level of expertise. Testing with an extreme groups to identify areas that can be improved. 
    
%     \item (Not sure) We can also ask some students or authors to fill out the datasheet for their experiments, and let us know what they think. 
    
% \end{itemize}
% We include a datasheet reporting on the crowdsourcing experiments associated to this paper. 
% If we don't run a crowdsourcing experiment, we can take one of our papers (and just say we took one paper of reference to keep it anonymised)





The second and third parts of the interview with experts focused on 1) assessing the \textit{clarity} and \textit{completeness} of the attributes in the taxonomy, and 2) how we could exploit this taxonomy and turn it a tool for reporting. Based on the taxonomy and feedback we received in the interviews, we derived a checklist for reporting crowdsourcing experiments,
%\footnote{\hll{The checklist can be found at \url{https://trentocrowdai.github.io/crowdsourcing-checklist/}. By publishing in a repository, we seek to encourage further discussion and participation from the community.}},
detailed in Appendix \ref{sec:checklist-table}.
% \footnote{We plan to publish the checklist on GitHub to motivate further participation from the community and facilitate materials to encourage its adoption.}.





The \textit{completeness} of the taxonomy makes sure the major ingredients of crowdsourcing experiments are well covered, while the \textit{clarity} concerns the interpretation and understanding of the attributes in the taxonomy. 
% 
%We found the taxonomy to be quite complete: the participants (6/10) suggested attributes that were already present in other parts of the taxonomy they did not assess. 
We found the taxonomy to be quite complete: the participants who identified missing elements (6/10) suggested attributes that were already present, but in other parts of the taxonomy they did not assess. 
%
One of the participants, \textit{P2}, suggested a ``when to stop'' attribute (not present in the taxonomy) for quality control, saying, \textit{``[...] when we are trying to collect quality data, we do not want to stop the task until we reach a threshold. Also, we might finish the task because we have already collected very good quality data"}. 
%
While we find this to be an excellent point, we argue that it is more related to data collection practices, for instance, to obtain data for ML, than for experiments in crowdsourcing. Therefore, we ultimately did not incorporate this aspect as an attribute in the taxonomy (besides, it could be covered by the existing post-task checks attribute).



\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/changes-exp.pdf}
  \caption{Example of updates we introduce to the attribute definitions in the taxonomy based on the feedback from the interviews (Experimental design dimension in this case), including the final framing as a checklist.}
  \Description{Example of updates we introduce to the attribute definitions in the taxonomy based on the feedback from the interviews (Experimental design dimension in this case), including the final framing as a checklist.}
  \label{fig:changes-exp}
\end{figure}





In general, the attributes were clear and relevant to the participants.
%
The suggestions of what attributes to add were used instead to improve the definition of the existing attributes, adding to the concrete feedback that focused on improving the definitions.
%
Figure \ref{fig:changes-exp} depicts some of the changes to the experimental design dimension and the final framing as a checklist.
%
Of the $39$ attributes in the taxonomy, $31$ were assessed by participants.\footnote{The requester dimension was not discussed with any of the participants. But aspects such as platform, ethics, and privacy were considered by some participants in the initial part of the interview.} 
% 
% the following comes from our "interviews sheet, feedback on attributes tab"
Participants provided feedback, on average, \hl{to 10 attributes (between 7 and 14), with an attribute being assessed by 2 to 4 participants}.
%
% the following comes from our "interviews sheet, feedback on attributes tab"
We noticed that \hl{16 attributes were clear ``as is", 9 were clear, but received suggestions to improve them, 3 were clear only after some clarification from the interviewer, and only 3 were not clear}.\footnote{We coded an attribute as clear if it was clear to all the participants who assessed it. To code as ``clear with suggestions'', ``clear after clarification'', or ``not clear'', we only expected at least one feedback to fall in these categories, prioritizing the not clear option.}




% framing
As for how we could exploit the taxonomy, we asked participants, \textit{``How do you think these aspects could be framed into a tool for reporting?''}. 
%
We clarified that the framing naturally depends on the intended usage and shared two examples. 
% The PRISMA checklist \cite{Prisma} that assesses the methodological rigor of systematic reviews. 
\hll{The first example was the PRISMA checklist \cite{Prisma} that assesses the methodological rigor of systematic reviews.}
And the other was datasheets found in the ML community, which are self-contained structured summaries of a dataset creation pipeline or model performance \cite{Gebru2019,DBLP:conf/fat/MitchellWZBVHSR19}.
%
The participants favored the checklist format \hl{(5/10)} over the datasheet alternative \hl{(1/10)}, while the rest did not explicitly mention a checklist but suggesting it based on their answer.



\subsection{Intended usage and adoption}

% format and % intended usage, help researchers be thorough and systematic on how they report their experiments, without suggestion where to put these details.

\hl{The intended usage of the taxonomy, how it is framed as a tool for reporting, and the adoption by the research community go hand in hand.}


\hl{A checklist format gives paper authors more flexibility to describe the different aspects of the experiments in the paper's main content and supplementary materials (weighing in typical page limits), indicating where an attribute is being described. We aim for the checklist to serve as a resource that guides researchers in what they report, helping them be thorough and systematic in communicating the details of their crowdsourcing experiments (i.e., serving as a reminder,  \textit{``when we are very deep into our data analysis part we forget the basic stuff that should be reported''}).}
%
Unlike a datasheet, a checklist is not self-contained, which was indicated by one of the participants, \textit{``To me, it is easier to see it as a report, with all the information on the same page [...]''}. 
%
While a self-contained summary as a supplementary material could be more convenient to readers, it demands more effort from authors since the main ingredients of the experiment would still need to be described in the paper, at least at a high level.
%
Guided by the feedback from the experts, we ultimately opted for the checklist format, considering that it helps authors report their experiments, while avoiding additional efforts, and readers to navigate the details of a crowdsourcing experiment.
%




% \hl{We aim for the checklist to serve as a resource that guides researchers in how they report, helping them be thorough and systematic in communicating the details of their crowdsourcing experiments.
% %
% We chose a checklist format as we believe it would put less burden on researchers. Besides, the checklist does not suggest where to describe the ins and outs of an experiment;  as conferences typically impose page limits, one could spread the reporting between the paper's main content and supplementary materials.
% %
% }





% challenges in adoption
% - evolving current practices in assessing experiments
% - burden put on researchers
% - convincing people to use
% so, how we incentivize this?

\hl{
During the interviews, the participants raised challenges associated with the adoption of a checklist --- \textit{``it all comes down to motivation''}.
%
%As simply put by a participant, 
One of this challenges was associated with the research community and the current practices around crowdsourcing experiments. As explained by a participant:
\textit{``you can probably check 30\% of those boxes and the paper will be published [...] no major motivations in the academic world other than your paper being published''}.
%
Adopting a checklist would go in tandem with evolving current community practices for assessing papers reporting on crowdsourcing experiments (as seen, for example, in the ML community, where reproducibility checklists are part of the submission/reviewing process\footnote{\url{https://neurips.cc/Conferences/2021/PaperInformation/PaperChecklist}}). However, we hope that bringing awareness about the potential issues of not standardizing practices can push the community in the right direction.
%
In response to this challenge, the experts highlighted the importance of growing adoption organically by making people aware of the benefits and lowering the barriers to adoption. As commented by the participants: \textit{``convince the people that these are the important things that you should follow''}, and \textit{``make researchers' life easier''}.
%And aligned to this, how to reduce the potential burden incurred on researchers adopting the checklist (i.e., \textit{``make researchers' life easier''}).
}




% how can we motivate its adoption
% \hl{
% The adoption of the checklist is also a relevant factor, as mentioned by some of the participants, this is linked to what motivates people to use it (e.g., \textit{``for people to really use it, then you need to put some incentive schemes.''}) or what we do to ease the adoption in the first place.
% }

% \begin{quote}
% \hl{\textit{It all comes down to motivation. 
% What is the motivation for a researcher who works in the crowdsourcing field to check all those boxes. Because, you can probably check 30\% of those boxes and the paper will be published and we all need to accept that no major motivations in academic world other than your paper is published. So what kind of extra motivation do you provide to the researchers. And maybe if you can clearly see that by checking all the boxes your paper will be published 17\% more often, it is some motivation. Which will not create motivations for the best researchers in the field. 
% If you want to create motivations for the best researchers in the field, you can make their lives easier. As a way to make their lives easier you say, hey tell me the platform, tell me the task ID, provide credentials, click ENTER, and a GitHub repository is created with all this information.}}
% \end{quote}



% \hl{We foresee promising avenues of future work that could facilitate the adoption of the checklist by the research community; in this work, we limited ourselves to starting the conversation towards reproducible crowdsourcing experiments. 
% %
% For example, one could focus on making researchers' lives easier via automatic tools that can derive most of the information from the underlying crowdsourcing platform.
% %
% }


\hl{
We foresee promising avenues of future work that could address these challenges and facilitate adoption by the research community. In this work, however, we limited ourselves to starting the conversation towards reproducible crowdsourcing experiments.
%
For instance, convincing people to adopt the checklist could be addressed by providing empirical evidence on how using the checklist aids reproducible results. Or making its usage so trivial that researchers just adopt it. For example, \textit{``As a way to make their lives easier, you say, hey, tell me the platform, tell me the task ID, provide credentials, click ENTER, and a GitHub repository is created with all this information''}.
}

==> CSCW 2021 - Reporting crowd experiments/sections/experiment.tex <==
% \section{Analysis: the case of sampling}

% time and demographic sampling and how these could swing the results.

==> CSCW 2021 - Reporting crowd experiments/sections/methods-checklist.tex <==
% \subsection*{Designing a checklist for reporting crowdsourcing experiments}
\subsection{Methods} \label{sec:methods-checklist}
%\subsection*{From a taxonomy to a checklist}


% We took the taxonomy and defined each of the attributes. The definitions were initially iterated on by two researchers. Then as part of the piloting phase, we took three papers from the papers of the authors and prepared the intended "reporting sheets". WE took their papers as it would not require further reading...
% The papers gave us a concrete example that we could discuss in the team. The discussions led to reframing of attributes, and deciding on what to include as part of the reporting. 
% Brainstormed on alternatives for the presentation. checklist vs datasheet..

% The checklist is the result of a process that involved three main steps: i) internally growing the taxonomy into a reporting sheet that was used in the internal assessment and pilots; ii) obtaining feedback from experts on the generic reporting sheet and views on alternatives strategies for reporting, and iii) developing and refining the checklist. We detail on this process below.


The checklist is the result of a process that involved three main steps: i) internally growing the taxonomy into a reporting sheet that was used in the internal assessment and pilots; ii) obtaining feedback from experts on the generic reporting sheet and views on alternatives strategies for reporting, and iii) developing and refining the checklist. 

Starting from the taxonomy, two researchers defined each of the attributes and prepared questions that would require authors to specify if and how each attribute is reported in a paper. These  definitions were then used as the initial template for piloting the reporting of three papers of the authors, leading to the definition of the first ``sheet'' for reporting. The sheet contained the attributes in our taxonomy as rows along with their definitions. 
We filled out the sheet with excerpts from the papers explicitly addressing the attributes in our taxonomy. This step gave us a concrete example that we could use to discuss among the team members. This discussion led to a reframing of attributes and deciding what to include as part of the reporting. 
The discussion also led to brainstorming alternatives for the presentation, where we considered datasheets \cite{Gebru2019,DBLP:conf/fat/MitchellWZBVHSR19} or checklists \cite{Prisma,MLReproducibilityChecklist} as potential options for guidelines for reporting.

% %Two researchers defined each of the attributes in the final taxonomy in terms of questions that check if and how these attributes are reported in a paper.
% %
% During the piloting phase described earlier (Section \ref{sec:methods-taxonomy}), we took three papers of the authors and prepared the intended ``sheet'' for reporting. 
% %
% % We selected these papers as it would not require further reading, and we were familiarized with the corresponding experiments.
% %
% The sheet contained the attributes in our taxonomy as rows along with their definitions. 
% %
% We filled out the sheet with excerpts from the papers explicitly addressing the attributes in our taxonomy. This step gave us a concrete example that we could use to discuss among the team members. This discussion led to a reframing of attributes and deciding what to include as part of the reporting.
% %
% The discussion also led to brainstorming alternatives for the presentation, where we considered datasheets \cite{Gebru2019,DBLP:conf/fat/MitchellWZBVHSR19} or checklists \cite{Prisma,MLReproducibilityChecklist} as potential options for guidelines for reporting.




% Part 2 - read aloud the descriptions of the attributes. reflect on relevance for reporting and clarify. 
% framing of the attributes, descriptions
% reporting resource alternatives
We focused Parts 2 and 3 of the interview with experts on assessing the definition of the attributes (as well as spotting missing ones) and collecting suggestions on how to present the guidelines for reporting.
%
Part 2 of the interview introduced participants with a portion of the final taxonomy (one or two dimensions). Participants (besides giving feedback on the relevance of the attributes and spot any missing one) were asked to read aloud attributes description and to assess and provide feedback on the framing.
% 
Part 3 asked, \textit{``How do you think these aspects of crowdsourcing experiments could be framed into a tool for reporting?''}, providing examples such as datasheets or checklists.

The answers collected from these parts of the interview were used, first, to improve the definitions of the attributes and, second, to derive the final form of the guidelines: a checklist for reporting crowdsourcing experiments. 
%We discussed the checklist with an expert in the field, where we collected additional thoughts on the idea of a checklist and suggestions for improvement (e.g., \textit{``What are your thoughts on the idea of a checklist for reporting crowdsourcing experiments? And do you have any general suggestions to give?''}). 
%We present the final checklist in Section \ref{sec:checklist}.



% final checklist
% discussed with an expert















% The previous step produced an initial taxonomy of crowdsourcing experiments. We continued updating the taxonomy considering three main reasons.
% %
% First, the taxonomy should focus on attributes directly associated with crowdsourcing, offloading general attributes to existing guidelines
% \footnote{Initially, the taxonomy considered attributes such as independent, dependent, and control variables. In later iterations, we omitted these attributes since they are well understood and covered in guidelines for experimental research.}.
% %
% Second, the focus should also be on practical and essential attributes for the reproducibility of experiments in crowdsourcing (e.g., instead of just describing the experimental conditions, authors should explain how these were mapped to tasks in crowdsourcing platforms).
% %
% And last, the attributes in the taxonomy should have a clear scope, avoiding ``unique cases'' or attributes that are too broad
% \footnote{For example, the taxonomy considered whether an experiment was ``synchronous'' (experiments with multiple phases where one phase's output serves as input to the next \cite{Mason2012,DBLP:conf/dagstuhl/GadirajuMNSEAF15}). We ultimately replaced this by introducing more specific attributes describing how the experimental design maps to crowdsourcing tasks and how they are executed.}.
% %
% The resulting taxonomy is the starting point to develop a checklist for reporting crowdsourcing experiments.






% Framing this taxonomy as a checklist also requires understanding how (and to what extent) crowdsourcing experiments report the attributes in the taxonomy.
% %
% We selected a random subset of $80$ articles from the $174$ papers reporting crowdsourcing experiments we previously identified. 
% %
% This subset consisted of 1) all the included papers from CHI, CSCW, and HCOMP conferences from 2018-2020 (\textbf{\color{red}X, Y, Z} papers, respectively), and 2) a random sample from 2013-2020 from other major conferences (skewing the sampling to recent papers).
% %
% Three researchers then analyzed these papers considering each of the attributes in the taxonomy: assessing the completeness (whether an attribute was reported), and how the attribute was reported in the paper. The process started with a small subset of \textbf{\color{red}X} papers to calibrate the level of agreement (\textbf{\color{red}Y\%}) and continued with the rest of the documents distributed equally among the researchers.
% %
% The results and further details of this step are described in Section \ref{sec:state}.




% %We developed an initial version of the datasheet based on the insights learned from analyzing the reporting of crowdsourcing experiments. 
% We started by framing the taxonomy as a datasheet for reporting experiments in crowdsourcing, leveraging on the insights learned from analyzing the state of reporting in crowdsourcing research. 
% %
% Each of the attributes in the taxonomy were defined as questions in the datasheet
% %
% The datasheet consists of dimensions, and each of the dimensions groups attributes that characterize crowdsourcing experiments. The datasheet is thus a table where each row is an attribute. An attribute is defined using questions that check if and how a concrete aspect of the crowdsourcing experiment is reported.
% %
% %We framed the items in the taxonomy as questions to support the process of reporting (and for readers to understand the design and operationalization of the experiment).
% %
% The datasheet was then validated with experts from the human computation community. We ran a series of semi-structured interviews to 1) understand what experts believe are the main ingredients of crowdsourcing experiments, 2) assess the relevance of the elements in the datasheet.
% %
% This process gave us valuable feedback to refine the datasheet and derive the version we propose in this work, presented in Section \ref{sec:checklist}.



% {\color{royalblue(web)}
% We validated the taxonomy of crowdsourcing experiments with experts from the human computation community ({\color{red}$\mathbf{N=9}$}).
% %
% The taxonomy was presented in tabular form, with attributes as rows and grouped in dimensions, defining an attribute using questions that check if and how a concrete aspect of the crowdsourcing experiment is reported.
% %
% We ran a series of semi-structured interviews to 1) understand what experts believe are the main ingredients of crowdsourcing experiments, 2) assess the relevance of the elements in the taxonomy.
% %
% This process gave us valuable feedback to refine the elements in the taxonomy and derive the checklist for reporting crowdsourcing experiments we propose in this work, presented in Section \ref{sec:checklist}.
% }










% para for the initial version of the datasheet and that we relied on semi-structured interviews to improved and derive the version we propose
% we started framing the taxonomy as a datasheet for reporting experiments
%we elaborated an initial version of the datasheet and gave a proper definition to the attributes in the taxonomy.
%we framed the taxonomy as a datasheet for reporting crowdsourcing experiments, associating each of the attributes with questions to help defining the attributes
%We mention that we validated the datasheet with experts from the community using semi-structured interviews where they commented on what they believe are relevant elements of crowdsourcing experiments and also evaluated the relevance of the elements in the proposed datasheet.







% Using an iterative process, the researchers updated the taxonomy in two phases, first testing the taxonomy against a small sample of crowdsourcing experiments from one of the conferences we considered and then updating the taxonomy to incorporate missing attributes.


% refined iteratively by testing the taxonomy, using considering papers from one of the conferences we consider, starting from a small sample of 5 papers and then continuing the process up to 15 papers, updating the taxonomy in the process until saturation was reached.


% we explain that we iteratively refined the taxonomy starting from a small sample (5) of the papers from a specific conference from the list. indicating that we performed a systematic analysis of this subset of papers according to our taxonomy


% a smaller scale of this procedure was published in [omitted]
% the result of this was published in [omitted] and we iterated on the taxonomy based on further feedback from reviewers.

% \bigskip
% % para
% 1. extracted attributes from small sample of papers from (1), (2), (3)
% 2. we organized attributes into an initial taxonomy
% 3. we iteratively refined this taxonomy using a random sample from (4) testing the taxonomy on the go, this process started from a small sample of 5 papers and proceed until saturation was reached
% 4. the result of this was published in [omitted] and we iterated on the taxonomy based on further feedback from reviewers.

% para
% 5. we hook the part currently in blue and we say that we now framed the taxonomy as a datasheet
% 6. we used semi-structured interviews to validate and improve the datasheet we propose in this paper.








% 1. introductory sentence and then we explain the 4 sources. followed by how we covered these four sources

% 2. explain how we elicited the initial version of the taxonomy

% 3. then we explain that we iteratively refined the taxonomy starting from a small sample (5) of the papers from a specific conference from the list. indicating that we performed a systematic analysis of this subset of papers according to our taxonomy

% 4. then we say the result up to this point was published and we iterated based on the feedback from the reviewers, framing this taxonomy now as a datasheet for reporting experiments in crowdsouricng

% 5. we mention that we validated the datasheet with experts from the community using semi-structured interviews where they commented on what they believe are relevant elements of crowdsourcing experiments and also evaluated the relevance of the elements in the proposed datasheet.





% Here we should describe the entire methodology. This includes

% - Taxonomy
% - Systematic analysis 
% - Datasheet






% {
% \bigskip
% \color{royalblue(web)}
% The taxonomy results of an iterative process that allowed us to modify the taxonomy from its initial version. Along this process, three main reasons motivated us to remove, add, split, or update the attributes of taxonomy. 
% %
% First, the taxonomy should focus on attributes directly associated with crowdsourcing, offloading the responsibility of general attributes to existing guidelines
% \footnote{Initially, the taxonomy considered attributes such as independent, dependent, and control variables. In later iterations, we omitted these attributes since they are well understood and covered in guidelines for experimental research.}.
% %
% Second, the focus should also be on practical and essential attributes for the reproducibility of experiments in crowdsourcing (e.g., instead of just describing the experimental conditions, authors should explain how these are mapped to tasks in crowdsourcing platforms).
% %
% And last, the attributes in the taxonomy should have a clear scope, avoiding ``unique cases'' or attributes that are too broad. 
% %
% For example, the initial taxonomy considered whether an experiment was ``synchronous''  as part of the \textit{Experimental design}
% \footnote{Synchronous experiments operate in multiple phases with the same or different sets of subjects, connecting the output of one phase as the input of the next \cite{Mason2012,DBLP:conf/dagstuhl/GadirajuMNSEAF15}}. 
% We then ultimately replaced this by introducing more precise attributes describing how the experimental design maps to crowdsourcing tasks and how these are executed.
% }

==> CSCW 2021 - Reporting crowd experiments/sections/methods-state.tex <==
% \subsection*{Analysing the state of reporting of crowdsourcing experiments}
\subsection{Methods} \label{sec:methods-state}

% full query used
% 18/06/2020 We obtained 586 records. And 458 using TITLE-ABS.
% TITLE-ABS-KEY(crowdsource OR crowd-source OR crowd-sourcing OR
% crowdsourcing OR "human computation" OR
% crowdsourc* OR crowd-sourc* OR m*cro-task OR m*crotask)
% AND
% TITLE-ABS-KEY(experiment OR "experimental design" OR stud* OR evaluation OR
% intervention OR analysis)
% AND
% TITLE-ABS-KEY(user* OR behavio* OR worker*)
% AND
% (CONF(CHI) OR CONF(HCI) OR CONF(CSCW) OR CONF(WWW) OR CONF(HCOMP) OR
% CONF(WSDM) OR CONF(CIKM) OR CONF(SIGIR) OR CONF(ICWE) OR CONF(IUI) OR
% CONF(UIST) OR CONF(ICWSM) OR CONF("Human Factors"))
% AND
% (LIMIT-TO (DOCTYPE ,  "cp"))
%
% DBLP, complementing some main conferences not indexed by Scopus (HCOMP)


% Sources
% Scopus 

% Inclusion criteria
% component of the query 
% crowdsourcing
% experiment


% Screening
% two researchers

% Metrics

% Sampling

% Process
% - initial analysis 15 papers / initial taxonomy (explained in the above section)
% - second round with the final taxonomy


%\ref{sec:query-screening}


The assessment considered the i) \textit{completeness}, referring to whether the attribute in question could be derived from the reported experiment, and ii) \textit{reporting style}, i.e.,  how the attribute was reported in the paper. We detail the process below. 

We started with a systematic search for scientific papers describing crowdsourcing experiments.
%
We iteratively refined a query for Elsevier's Scopus database to cover a wide range of crowdsourcing experiments in computer science and ensure the taxonomy fits well with a broad range of experiments.
The query consisted of keywords covering different usages or words associated with \textit{crowdsourcing} (e.g., ``crowd-sourcing'', ``micro-task'', ``human-computation'') and \textit{experiments} (e.g., ``experimental design'', ``study'', ``evaluation'', ``analysis'', ``intervention'').
We also limited the search space to papers published in major conferences (e.g., CSCW, CHI, IUI, UIST, HCOMP) between January 2013 and June 2020, \hl{excluding journal papers from the query to keep the search space focused}. 
%
We complemented this search by downloading from DBLP the list of papers in the proceedings of relevant conferences not indexed by Scopus.
%

The search identified a total of $670$ candidate papers. These papers were screened by two researchers to include papers describing experiments or user studies engaging crowd workers as subjects through a crowdsourcing platform. We excluded experiments leveraging on existing crowdsourced datasets, engaging workers in a role not related to the evaluation, experiments in laboratory settings, \hl{purely qualitative studies (e.g., surveys)} and experiments where crowd workers did not come from an open call to a crowdsourcing platform but rather from a more restricted environment. 
The screening started with a random subset of $50$ papers to calibrate the aforementioned eligibility criteria between the researchers, and then proceeded with the researchers screening independently the rest of the documents (the researchers agreed on 94\% of the decisions in the set of 50 papers, resolving disagreements by consensus). 
This process identified \hl{$172$} papers reporting crowdsourcing experiments. We refer readers to the Appendix \ref{sec:query-screening} for more details on the search and screening process, including the query and eligibility criteria.



% From the pool of \hl{$172$} crowdsourcing experiments, we selected a sample of $80$ experiments, representing the diversity of efforts across as well as recent efforts in main relevant venues. Thus, the sample consisted on 1) a random sample from all conferences by year of publication since 2013; and 2) all experiments published in CHI, CSCW and HCOMP conferences since 2018. We designed the second sample to reflect recent efforts in reporting crowdsourcing experiments coming from a more mature understanding of biases in crowdsourcing, and subject to high technical standards. 



%
The analysis then proceeded in three phases that aimed at assessing the reporting of experiments in terms of the taxonomy of relevant crowdsourcing experiment attributes. It started with a small sample of 15 papers, as explained in the above section, to iteratively refine the initial taxonomy and the assessment metrics. 
%
\hl{Second, to calibrate the interpretation of the taxonomy and the assessment metrics, a subset of 40 papers ($\sim$25\% of the total number of included papers) was analyzed by three researchers, resulting in an average agreement of 90\%. The researchers assessed all the taxonomy attributes for the same set of papers, considering as a match if they agreed on the completeness value (i.e., the presence of an attribute in a paper).
}
Finally, the rest of the documents were distributed equally among the researchers and assessed independently. Only one experiment was analyzed per research article, and in the case of papers reporting on multiple experiments, one experiment was randomly selected.   
\hl{Any doubts emerging during the independent tagging were flagged by the researchers for discussion and resolved by consensus. }




The analysis followed a meticulous procedure where the researchers leveraged on their experience (and the input from experts) to assess the completeness of the attributes of an experiment,  evaluating only those applicable to \hl{ i) the type of experiment reported in the paper, and ii) the objective of the study}. This approach was followed as it was clear from our pilots, interviews with experts and our own experience that not all attributes were relevant for each experiment. 
%
\hl{
With these criteria, the researchers ended up applying 26 of the 39 attributes in all cases, with the other 13 deemed not applicable (N/A) depending on the type and goal of the experiment.
%The researchers only considered 13 of the 39 attributes in the taxonomy as potentially not applicable (N/A) based on an experiment's goal, with the rest of the attributes always applicable. 
We found that, on average, four attributes were N/A and that 80\% of the papers in our analysis had at most six N/A attributes.
%
Notice that we adjusted the total number of attributes on a per-paper basis, excluding the N/A attributes. Similarly, the percentages we report for each attribute in Figure \ref{fig:state} are also adjusted by removing N/A cases. We refer readers to Appendix \ref{sec:applicability-attr} for further details.
}

%
Taking the quality control attribute \textit{In-task checks} as a concrete example, the researchers first checked whether the paper explicitly mentioned any quality checks performed during the task (e.g., gold items, attention checks), and to the best of their abilities assessed whether they were indeed applicable for the particular type of experiment (e.g., the experiment studied cheating behavior where in-task checks would not make sense). Researchers then continued by checking if the details relevant to this quality control check could be derived from the description, even if the papers did not explicitly describe it (and in this case, it was counted as ``implicit reporting’’).
%
\hl{There are also some attributes with a ``directional association''. For example, we considered the interface and instructions as complete if the paper provided the source code (and, for example, omitted screenshots of these). Likewise, if \textit{informed consent} was explicitly reported, we considered as complete the \textit{participation awareness} attribute.}


\hl{
The assessment of the reporting covered not only the main content of the paper but also the appendix, supplementary materials and any source code or repository associated to the paper. To identify these additional sources, the researchers checked for links referenced or cited in the paper, as well as the official page of the paper in the publisher's website.
%As an additional example, for an attribute such as the \textit{task interface}, researchers checked for descriptions and screenshots of the task considering the main content of a paper, appendices, supplementary materials, and the source code (if made available in an online repository). If only a textual (and partial) description of the task interface was provided, researchers coded this case as ``implicit reporting''.
}
%
This procedure was followed to assess the completeness of all the attributes in the taxonomy.

==> CSCW 2021 - Reporting crowd experiments/sections/methods-taxonomy.tex <==
\subsection{Methods} \label{sec:methods-taxonomy}


We consider four sources to elicit the taxonomy: i) guidelines for research experiments in general and specific to crowdsourcing experiments, ii) features available in crowdsourcing platforms to support the deployment of experiments,  iii) scientific papers describing crowdsourcing experiments, and iv) interviews with experts.
%
With these sources we aim to convey in the taxonomy the landscape of elements taking part in crowdsourcing experiments: elements from experimental research, those inherent to crowdsourcing, and what features platforms offer.




We started by identifying relevant attributes from existing guidelines. For this, we took a small seed of well-known guidelines for experimental design and crowdsourcing \hl{\cite{Gergle2014,Mahmood2015,Porter2020,Mason2012,DBLP:conf/dagstuhl/GadirajuMNSEAF15} and expanded it through snowballing and  keywords search using Google Scholar (\textit{``crowdsourcing + guidelines''}, \textit{``crowdsourcing + best practices''}, \textit{``crowdsourcing + recommendations''}, and \textit{``crowdsourcing + reporting + experiment''}) and screening the results based on title.}
%
This perspective was complemented with the analysis of practical task design attributes \hl{available in a example micro-task platform, Toloka~\footnote{\url{https://toloka.yandex.com/}}, which provides all common features for managing microtask crowdsourcing}.
%
\hl{The analysis of platforms' features allowed us to ground attributes to practical "knobs" that researchers need to consider to operationalize their experiments, and that often fall into assumptions (e.g., training steps, mapping of experimental design to concrete micro-tasks).}
%
Leveraging these sources, two researchers extracted an initial set of attributes \hl{(e.g., task interface, task instructions, compensation, crowd demographics, research design, random assignments, platform used, fair payments, among others)} in a spreadsheet to form an emerging list. The two researchers then jointly discussed and organized these attributes into six dimensions as depicted by the top-level entries in Figure \ref{fig:taxonomy}. 



\hl{This organization of attributes required the two researchers to iteratively group the attributes identified in the seed of papers and selected crowdsourcing platform around common themes
(e.g., dimensions like \textit{pool of participants}, \textit{workers}, and \textit{study participants} were unified as the \textit{crowd} dimension). This was followed by an analysis of the initial set of attributes extracted, merging (whenever possible) equivalent attributes from different sources  (e.g., \textit{task template} and \textit{task UI} as \textit{task interface}).
}
%
\hl{Notice that during this process, the researchers defined the semantics and scope of each of the six dimensions, as well as that of the individual attributes.
We should stress, however, that our aim is on the comprehensiveness in terms of the attributes we identified and not the way we organized these into dimensions, which is a specific way of viewing things. 
For example, we include the demographics attribute under Outcome, as we define this dimension as the one capturing the \textit{results} of the different aspects of the crowdsourcing process (including the recruitment, application of quality control techniques, etc). Under different semantics, one might put demographics under the Crowd dimension, but we defined this dimension as the one capturing attributes and mechanisms to identify and sample participants from the Crowd.
}

This initial taxonomy was then refined by analyzing and piloting the extraction of relevant crowdsourcing experiment attributes from a list of research papers reporting crowdsourcing experiments. The process of identifying these papers is described in Section \ref{sec:methods-state}, as part of the analysis of the state of reporting. From this list, we took a random sample of 15 papers published in the last eight years, which we drafted incrementally until we reached saturation \cite{saunders2018saturation}. 
In this piloting phase, researchers took note of the applicability of the attributes for certain types of experiments, new attributes not initially considered, as well as attributes to be discarded or merged. These observations were discussed and addressed jointly by the two researchers.

We then further refined and validated this taxonomy with the input from crowdsourcing experts. To this end, we used the input collected in Part 1 and (some bits of) Part 2 of the semi-structured interviews with experts. The goal was to tap into their experience to identify, through different trigger questions, relevant attributes that we might have missed. 
%
We leveraged their input by inquiring about their experience running and designing crowdsourcing experiments (e.g., \textit{``What design choices you found to be more critical, possibly affecting experiment outcomes?"}), reporting or trying to replicate experiments (e.g., \textit{"What aspects you deem relevant and should be reported?"}), and their own experience reading or reviewing papers (e.g., \textit{"What aspects do you find to be typically under-reported or poorly reported?"}). In doing so, the interviewer would bring up only the top level dimensions (e.g., quality control or task design) if they were not discussed by the participant. We avoided providing any details about specific attributes so as not to bias the participants towards our taxonomy.
%
Then, Part 2 introduced a portion of the taxonomy (one or two dimensions) and asked participants to assess the relevance of the  attributes and to suggest any missing one.
%



\hl{
Transcripts were organized around the trigger questions in a document, where the interviewer highlighted excerpts touching on crowdsourcing attributes (e.g., \textit{``[...] depending on the \underline{design of the interface} you might get wide results.''}). These excerpts were then moved to a spreadsheet for analysis.
%
The interviewer then coded the excerpts with the associated attribute if covered by our taxonomy or flagged them for discussion otherwise.
%
The two researchers then discussed the coded excerpts and assessed whether i) the attribute was relevant to the scope of the taxonomy, ii) the scope and name of an attribute had be updated to cover a more general case, iii)  the scope of the attribute had to be limited to account for scenarios where an attribute is not applicable.
}


The inclusion criteria we used to refine the taxonomy considered three main reasons.
%
First, the taxonomy should focus on attributes directly associated with crowdsourcing, offloading general attributes to existing guidelines.\footnote{Initially, the taxonomy considered attributes such as hypotheses, independent, dependent, and control variables. In later iterations, we omitted these attributes since they are well understood and covered in guidelines for experimental research.}
%
Second, the focus should also be on practical and essential attributes for the reproducibility of experiments in crowdsourcing (e.g., instead of just describing the experimental conditions, authors should explain how these were mapped to tasks in crowdsourcing platforms).
%
And last, the attributes in the taxonomy should have a clear scope, avoiding ``unique cases'' or attributes that are too broad.\footnote{For example, the taxonomy considered whether an experiment was ``synchronous'' (experiments with multiple phases where one phase's output serves as input to the next \cite{Mason2012,DBLP:conf/dagstuhl/GadirajuMNSEAF15}). We ultimately replaced this by introducing more specific attributes describing how the experimental design maps to crowdsourcing tasks and how they are executed.}
%
The resulting taxonomy is the starting point to develop a checklist for reporting crowdsourcing experiments.






==> CSCW 2021 - Reporting crowd experiments/sections/related.tex <==
\section{Related work}

\subsection*{Guidelines for reproducibility and reporting of scientific studies}


Reporting and reproducibility are at the heart of science.
Experiments allow researchers to manipulate a set of variables to test their influence into another group of variables of interest \cite{shadish2002experimental}. 
%
Guidelines for reporting scientific studies emerge from the observed variance in the methodological rigor associated with the studies. 
Indeed, the output of experimental research is only meaningful as long as it is reproducible \cite{DBLP:conf/www/Paritosh12}. This property guides the adopted methodology, as well as how this methodology and the results are communicated.




For example, in the study and synthesis of scientific results obtained via systematic literature reviews (SLRs), papers adhere to precise reporting guidelines that describes the (systematic) approach to investigating a problem as discussed in the literature.
% 
The existence of study and study report protocols is what gives systematic reviews its methodological rigor, avoiding issues like a biased selection of clinical outcomes \cite{ChanEmpirical2014}. 
%
In this context, the PRISMA \cite{Prisma} guidelines propose a checklist to support the preparation and reporting of SLRs, making sure that such protocols exist and are reproducible.







In medicine, randomized control trials (RCTs) are the gold standard methodology to evaluate medical interventions. In this regard, guidelines like the CONSORT statement \cite{schulz2010consort} help authors properly report their RCTs and avoid potential issues resulting from the lack of methodological rigor (e.g., biased outcomes).










\subsection*{Guidelines in crowdsourcing contexts}


Research has shown how crowdsourcing could be leveraged in a wide range of tasks and domains (e.g., from labeling data for ML \cite{DBLP:conf/emnlp/SnowOJN08,DBLP:conf/cvpr/SorokinF08} to serving as a platform for experimental research \cite{DBLP:journals/sigkdd/MasonW09,Paolacci2010RunningEO,Crump2013}). 
%
Existing guidelines and best practices focus on how to run experiments in crowdsourcing environments successfully, proposing strategies to overcome common pitfalls found in crowdsourcing platforms \cite{DBLP:conf/chi/KitturCS08,DBLP:conf/icwsm/RogstadiusKKSLV11,Mason2012,Chandler2013}.
%
However, how to properly report crowdsourcing experiments has, to the best of our knowledge,  been somewhat overlooked. Our work complements experimental research in crowdsourcing by providing guidelines to aid researchers in reporting crowdsourcing studies.




Crowdsourcing acts as a surrogate to traditional participant samples, but with additional challenges that are not present in traditional experimental settings.
%
The quality of the contributions provided by crowd workers is a major concern due to the diversity in worker skills and the level of commitment crowd workers put into the task \cite{DBLP:conf/dagstuhl/GadirajuMNSEAF15}. Many quality control mechanisms have been proposed (e.g., see \cite{DBLP:journals/csur/DanielKCBA18} for a review) as well as studies analyzing performance as a function of internal and external factors, showing that intrinsic motivation could help in increasing the performance of workers \cite{DBLP:conf/icwsm/RogstadiusKKSLV11}.
%
Factors related to the design of the task could also contribute to obtaining subpar responses. Poorly written task instructions could misguide workers and result in low-quality work \cite{DBLP:conf/hcomp/WuQ17,DBLP:conf/cscw/KitturNBGSZLH13,DBLP:conf/ht/GadirajuYB17,DBLP:conf/naacl/LiuSBLLW16}. 
%
In contrast, enhanced interfaces may facilitate the job of crowd workers and aid these to improved performance \cite{DBLP:conf/chi/SampathRI14,Wilson2016WWW,ramirez2019,RamirezBMC2019}, as well as adequately limiting the time to judge can accelerate task completion without compromising the quality of the results \cite{maddalena2016crowdsourcing}.



Another challenge relates to how we operationalize an experimental design in a crowdsourcing platform. %and make sure it is reproducible.
%
\hl{As opposed to laboratory settings, there is an inherent lack of control over the participants of crowdsourcing (and online) experiments that represents a concern to researchers, amplified by the absence of built-in support from crowdsourcing platforms \cite{DBLP:conf/chi/KitturCS08}.}
%
%The lack of complete control over the participants is a concern, amplified by the absence of builtin support from crowdsourcing platforms \cite{DBLP:conf/chi/KitturCS08}.
%
Random assignment, although simple in principle, is not straightforward to implement. Using multiple tasks to map different experimental conditions is a typical approach \cite{DBLP:conf/www/HoSSV15}; however, self-selection effects could arise due to participants preferring a subset of the conditions over others.
%
And ensuring that new workers arrive in the experiment is crucial to proper random assignment \cite{Mason2012,Chandler2013}, avoiding scenarios where workers participate multiple times in longitudinal studies or experiments that must run multiple times.
%
The characteristics of the platform should also be kept in mind.
%
The underlying demographics associated with the active workers \cite{DBLP:conf/wsdm/DifallahFI18} play an important role since differences in the conditions could be attributed to differences in the population of workers rather than the conditions themselves \cite{Qarout2019PlatformRelatedFI}.








Recent guidelines also safeguard the ethics behind crowdsourcing experiments.
%
Previous literature on humanizing crowd work pointed out relevant ethical issues present in common crowdsourcing practices (e.g., initially, crowdsourcing was seen as a ``cheap labor market'', as briefly reviewed in \cite{DBLP:conf/chi/BarbosaC19}). One aspect of this regards to accurate and fair task pricing \cite{Whiting2019FairWC}, which previous work has shown to impact the number of contributions produced by workers \cite{DBLP:journals/sigkdd/MasonW09}, the quality of their work \cite{DBLP:conf/www/HoSSV15}, and being a relevant aspect from an ethical perspective.
%
Another aspect concerns privacy, especially if some properties of the workers are being requested as part of the experiments \cite{Mason2012}.











As crucial as successfully conducting experiments in crowdsourcing environments, it is to make sure crowdsourcing experiments are reproducible \cite{DBLP:conf/www/Paritosh12,Qarout2019PlatformRelatedFI}.
%
In this regard, proper reporting of the methodology, operationalization, and results of crowdsourcing experiments plays a relevant role. 
%
Surprisingly, guidelines for reporting crowdsourcing experiments have received little attention even though underreporting is a serious concern in science, and crowdsourcing is no exception \cite{Buhrmester2018}.
%
Existing literature has identified how current studies fail to adequately report the methodology behind their crowdsourcing experiments, showing that most of the papers tend to omit information about worker qualifications, task design, rejection or validation criteria \cite{Porter2020,Ramirez2020DrecCSCW}.
%
These efforts propose templates for reporting studies, capturing essential aspects of crowdsourcing experiments.
%
However, these works are so far focused on specific use cases and platforms (data collection for social sciences in Amazon Mechanical Turk \cite{Porter2020}), or are still work-in-progress \cite{Ramirez2020DrecCSCW}.


Existing guidelines cover very well how to effectively leverage crowdsourcing in different contexts, but it has barely grappled with how to report crowdsourcing studies properly.
%
We aim to fill this gap by proposing guidelines for reporting the relevant aspects of crowdsourcing experiments. 
%
% \hl{As a starting point, our work leverages on the preliminary taxonomy proposed in \cite{Ramirez2020DrecCSCW}, we then redefine it based on an iterative process consisting of a large-scale analysis of papers reporting crowdsourcing experiments, 171 articles from the literature, and by drawing from feedback from experts in the field. In addition, we grow this taxonomy into a checklist to aid how researchers report experiments in crowdsourcing.}
\hll{As a starting point, our work leverages on the preliminary taxonomy proposed in \cite{Ramirez2020DrecCSCW}. 
The final taxonomy we propose differs from DREC's in terms of validation and scope of the attributes.
The validation stems from a mixed approach involving a large-scale analysis of papers reporting crowdsourcing experiments, 171 articles from the literature, and feedback from experts in the field.
%
% This approach helped us to scope down and refine the taxonomy to only attributes relevant to crowdsourcing experiments, leaving off attributes that are well-understood and covered in guidelines for experimental research (e.g., in the final taxonomy, the \textit{experimental design} dimension has 7 attributes vs. 13 in DREC). 
This approach helped us to scope down and refine the taxonomy to only attributes relevant to crowdsourcing experiments, leaving off attributes that are well-understood and covered in guidelines for experimental research 
\footnote{\hll{In the final taxonomy, the \textit{experimental design} dimension has 7 attributes vs. 13 in DREC. Here, the taxonomy omits attributes covered in guidelines for reporting study design and protocols (e.g., \cite{Gergle2014}). Likewise, the \textit{outcome} dimension, for example, omits the \textit{data analysis} attribute in DREC, as this is addressed by guidelines for reporting statistics (e.g., \cite{APA6thEDITION}).}}.
%
The final taxonomy also avoids narrow or too broad attributes (e.g., DREC's \textit{synchronous} and \textit{data analysis} attributes, respectively), as well as having attributes that can collapse into a single one (e.g.,  \textit{reputation} and \textit{environment} attributes are now part of the \textit{target population}).
%
In addition, our mixed approach allowed us to shape the final taxonomy into a checklist to aid how researchers report experiments in crowdsourcing.
}



% - diff in terms of scale 15 vs. 171
% - the taxonomy here is validated
% - the taxonomy is scoped to crowdsourcing, leaving off attributes for experiments in general
% drec: 45 attrs
% here: 37










==> CSCW 2021 - Reporting crowd experiments/sections/reporting.tex <==
\section{Analyzing the state of reporting} \label{sec:state}

To study the state of reporting we surveyed \hl{171} crowdsourcing experiments from the literature, and assessed them on the basis of the relevant crowdsourcing experiment attributes from our taxonomy. 
%
We used the attributes to assess the \textit{completeness} and \textit{reporting style} used in communicating the attributes. By doing this, we aim to shed light on the level of reporting in current practices. In the following, we describe the methodology and results.




\input{sections/methods-state}


\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/descriptive-stats.pdf}
  \caption{\hl{Some descriptive statistics of the 171 papers we analyzed. a) The distribution of papers by completeness, i.e., the proportion of attributes reported. The dashed line indicates the median. b) The distribution of papers based on their length (\textit{``d''}stands for double-column and \textit{``s''} for single-column format. c) The distribution of papers based on their year of publication.}}
  \Description{Some descriptive statistics of the 171 papers we analyzed. a) The distribution of papers by completeness, i.e., the proportion of attributes reported. The dashed line indicates the median. b) The distribution of papers based on their length (\textit{``d''} stands for double-column and \textit{``s''} for single-column format. c) The distribution of papers based on their year of publication.}
  \label{fig:descriptive}
\end{figure}



\subsection{Results}

\hl{We analyzed 171}\footnote{\hl{One paper was excluded from the analysis as the full-text was not available to the researchers.}} papers published in major venues to understand how (and to what extend) crowdsourcing experiments are reported. 
%
As mentioned previously, we used the attributes in the taxonomy to guide the analysis, assessing the completeness (e.g., \textit{is the attribute addressed?} And, \textit{is it explicitly reported?}), and the reporting style used in communicating the attributes (e.g., using screenshots, a figure, etc.).
By doing this, we seek to elucidate the level of reporting in current practices. 
%
\hl{We limited the analysis to 38 attributes, excluding the \textit{implemented features} attribute.\footnote{\hl{It is important to report on the features implemented to operationalize an experiment, but we found it difficult to reliably determine whether this attribute was applicable and being reported when analyzing the papers.}}}
%
% \hl{Figure \ref{fig:completeness-hist} depicts the distribution of papers based on the percentage of attributes reported. The papers reported, on average, 49.9\% of the attributes (19 attributes), with 89 of the 171 articles reporting at least 50\% of the attributes. 
% }
%
%\hl{Figure \ref{fig:state} summarizes the analysis for each of the six dimensions in the taxonomy.}






% 2013 2014 2015 2016 2017 2018 2019 2020 
% 20   17   20   32   22   27   29    4 


%\hl{Figure \ref{fig:state} summarizes the analysis for each of the six dimensions in the taxonomy.
\hl{Figure \ref{fig:descriptive} depicts some descriptive statistics of the papers we analyzed. The papers reported, on average, 49.9\% of the attributes (19 attributes), with 89 of the 171 articles reporting at least 50\% of the attributes. 
%
Of the papers analyzed, 89 of 171 were published between 2013 and 2016, and 82 of 171 were published between 2017 and June of 2020. 
%
Most of the documents (167 papers) were in double-column format and four in single-column format. The majority (143/171) are long articles (defined as those with \#pages $\ge$ 6 double-column, with 3 papers of 12+ pages long in single-column format), and 28 are short (\#pages $<$ 6 double-column, and one paper with 8 pages single-column). 
}



\hl{
We analyzed the level of reporting by year and length to contrast past and recent reporting efforts and differences based on paper length due to more pages available. 
%
We did not observe a clear pattern of recent papers addressing more attributes when compared to older ones, but we noticed an interesting trend of increasing reporting in longer documents. 
%
As for the attributes in our taxonomy, in 32/38, we noticed an increase in the percentage of papers reporting them, with relative differences of up to $3x$. However, the reporting was low, as the number of attributes covered by at least $50\%$ of the papers was $14$ for short and $16$ for long. 
%
Overall, the median completeness for short papers was $42.4\%$ and $51.5\%$ for long. 
%
Also, we did not observe any trend in the usage of supplementary materials to cover the lack of space, as only 15/171 papers provided supplementary material\footnote{\hl{The supplementary material included screenshots of the task (7/15), task source code (5/15), input dataset (8/15), output dataset (8/15), and other details related to data analysis (e.g., scripts, notebooks). Most of this material was provided as external links to a code repository (9/15) or document (3/15), two were in the appendix, and one was found via the publisher's digital library (video presentation).}}. Of these, three were short papers. 
%
A detailed breakdown of the results by year and length can be found at \url{https://tinyurl.com/ReportingState}.
}

%up to three times

% -----------------
% We have not identified a clear pattern based on the year of publication.

% completeness by len
% Length	Median	Mean	Papers
% short	0.424	0.4190000	28
% long	0.515	0.5156434	143

% In 32/38 attributes we noticed an increment of the percentage of papers reporting it, with this difference ranging between X% and Y%.
% -----------------


% supp materials
% 15 in total, 12 long, 3 short




%The reason to look at the results by year is to contrast past and recent efforts in reporting crowdsourcing experiments. The underlying assumption was that recent papers would address more attributes in our taxonomy. However, overall, we did not observe a clear pattern supporting this assumption.

%\hl{We observed an interesting trend of increasing reporting in longer documents.
%
% Most of the documents (167 papers) were in double-column format and four in single-column format. The majority (143/171) are long articles (defined as those with \#pages $\ge$ 6 double-column, with 3 papers of 12+ pages long in single-column format), and 28 are short (\#pages $<$ 6 double column, with one paper with 8 pages single-column format). 
%
% by year no clear pattern but by len we found diff by attr and %completeness by paper. so mention this part here and then say that interesting differences will be discussed.
%
%As part of our analysis, we will discuss interesting and relevant differences on the reporting level based on the year of publication and paper length. A detailed breakdown of the results by year and length can be found at \url{https://tinyurl.com/ReportingState}.
%}


\hl{Figure \ref{fig:state} summarizes the analysis for each of the six dimensions in the taxonomy. In the following, we discuss the results for the attributes in each dimension, and when necessary, we will touch on interesting and relevant differences on the reporting level based on the year and length.}






% Figure \ref{fig:state} summarizes the analysis for each of the six dimensions in the taxonomy. 
% Section \ref{sec:methods-state} described the papers analyzed come from two pools, a random sample of 48 papers from 2013-2020 (\textit{random} for short) and all 32 articles from CSCW/CHI/HCOMP 2018-2020 (\textit{main} for short). For the analysis, we split \textit{random} further into \textit{pre-2018} (37 papers published between 2013-2017), and \textit{recent} (11 papers published between 2018-2020).
% %
% This split is intended to contrast past and recent efforts in reporting crowdsourcing experiments. The underlying assumption was that recent papers would address more attributes in our taxonomy. However, overall, we did not observe a clear pattern supporting this assumption, but we will discuss interesting and relevant differences when necessary (see Appendix \ref{sec:state-by-pool} for detailed results).
% %
% The majority (69/80) of the analyzed documents are long articles (pages $\ge$ 7 double-column, with two papers of 13 pages long in single-column format), and 11 are short (pages $<$ 7 double column).





\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/state-171.pdf}
  \caption{The state of reporting, based on the attributes in the taxonomy, for a \hl{set of 171} papers describing crowdsourcing experiments published in major venues. \hl{The number of papers to which the attribute applied is indicated in parenthesis, and in boldface, the percentages of papers reporting on it (explicitly and implicitly).}}
  \Description{The state of reporting, based on the attributes in the taxonomy, for a set of 171 papers describing crowdsourcing experiments published in major venues.}
  \label{fig:state}
\end{figure}





% experimental design
\subsubsection*{\textbf{Experimental design}} Despite being the cornerstone of crowdsourcing experiments, the explicit reporting of experimental design attributes is for the most part shallow and unclear, as indicated by the low levels of explicit as well as high levels of unclear reporting -- the highest among the rest of the dimensions.
%
Overall, 4/7 attributes in the experimental design dimension -- those defining the design, mapping and execution of the experiment in the crowdsourcing platform -- are reported explicitly by \hl{52.4\% to 65.2\%} of the papers, representing the highest reported attributes for this dimension. When the experimental design is relatively simple and straightforward to map to a crowdsourcing environment (e.g., a within-subjects design mapping to a single crowdsourcing task), these four attributes can be derived with sufficient confidence, as indicated by the \hl{16.4\% to 24.7\%} of implicit reporting. But as soon as the design is more complex (e.g., a mixed design with multiple conditions and no clear hint on how these map to tasks), this is no longer the case, \hl{as indicated by the 0.6\% to 7.7\% of shallow and unclear reporting.} 

%                               Attribute value.Y.E value.Y.I value.U value.N
% 15                   Execution timeframe     0.146     0.018   0.000   0.836
% 16                                Pilots     0.275     0.029   0.006   0.696
% 17                     Returning workers     0.271     0.096   0.054   0.633
% 18  Execution of experimental conditions     0.524     0.214   0.077   0.262
% 19 Allocation to experimental conditions     0.592     0.165   0.071   0.243
% 20                         Input dataset     0.652     0.164   0.070   0.184
% 21   Experimental Design to task mapping     0.612     0.247   0.065   0.141



In terms of reporting style, the input dataset allowed for the richer set of approaches, compared to the rest of the attributes that were reported mostly in text.  A \hl{65.2\%} of the papers reported the actual input dataset used in the tasks given to workers, providing references or a link to an external site.  
However, some papers only indicated the process that was followed to prepare the input dataset and that would allow a researcher to construct a dataset of similar characteristics (which we coded as implicit, \hl{16.4\% of papers}). In \hl{two cases}, the provided link was no longer reachable, which brings a different issue: reporting links to supplementary materials that do not survive the ``test of time.''

Under-reported details include whether pilots were performed, if and how returning workers were controlled, and the experiments' execution timeframe. Pilots help tune the design of the experiment; however, it was only reported by \hl{27.5\%} of the papers. Returning workers, applicable depending on the design and how it is mapped, was reported by very few papers (only \hl{27.1\%}). Similarly, only \hl{14.6\%} of the papers reported the period in which the experiment run.
%
%No clear trend was observed when analyzing the results for each of the pools of papers.
\hl{For long papers, all of the attributes show an increase in explicit reporting, with relative differences of up to $2x$. But, only 4/7 attributes are reported by at least 50\% of papers against 3/7 in short articles.}








% crowd
\subsubsection*{\textbf{Crowd}} 
% papers describe what target population is but they tend to omit how they sample workers that will participate in their studies.
In general, \hl{62\%} of the papers explicitly reported properties characterizing the target population of workers suitable for the study, with \hl{2.3\%} of the papers implicitly suggesting what constitutes the target population \hl{(e.g., based on the goal of the study, we inferred that the task was open to everybody in the selected platform)}. Ultimately, this information was not clear in \hl{2.3\%} of the analyzed articles.
%
The exact mechanism used to sample a diverse and representative set of participants was reported in only \hl{12.9\%} of the papers (e.g., one possible strategy would be to sample systematically at different times of the day). \hl{In 3.5\% of the papers, this information was not explicitly addressed, but we derived by inference, which we coded as implicit (e.g., by providing the name of an external tool, by an auxiliary task to reach potential participants first).}
%
The above comes at a surprise, given the highly diverse and changing nature of crowd workers, and the potential influence of participants' characteristics and associated environment in task performance. In terms of reporting styles, these attributes are embedded in the paper as text. 
%No particular trend was observed when comparing the results by paper pools.
\hl{The target population was reported by $64.3\%$ of long papers vs. $50\%$ for short. And while the sampling mechanism was largely under-reported, it also shows an increase (14\% for long, and 7\% for short)}.

%           Attribute value.Y.E value.Y.I value.U value.N
% 5 Sampling mechanism      12.9       3.5     0.6    83.6
% 6  Target population      62.0       2.3     2.3    35.7




% task
 \subsubsection*{\textbf{Task}} The task dimension is relatively well covered.
%
The type of task, the reward strategy, and how the task looks like (including the instructions) are the attributes reported by most of the papers. 
%Intuitively, 100\% of the papers reported the task type, and 
Of the papers analyzed, \hl{83.6\%} of them explicitly described the strategy used to reward workers for their contributions (almost all papers described monetary compensations as the reward strategy, except for \hl{three articles} resorting to volunteering).
%
The task interface was explicitly reported by \hl{66.1\% of the papers}.
%
Some articles (\hl{17.5\%}) did not explicitly include a screenshot of the task and instead described it partially in text (which we coded as implicit).
%
When reported, the interface is mostly depicted using screenshots and just a handful of papers \hl{(4.1\%) provided the actual source code of the interface, and in two cases the link provided was no longer available (coded as implicit)}.
%
But even relevant information such as the instructions is reported explicitly by \hl{61.4\%} of the papers. The instructions can be reconstructed from \hl{partial screenshots and textual descriptions in some cases (19.3\% of the papers)}. 
%
Explicit time constraints are reported in only \hl{38\%} of the papers.
%
%Across the pool of samples we consider, only the reporting of the task interface attribute seems to have improved over the years (62.2\% in \textit{pre-2018} papers, and 81.3\% in \textit{main}).
\hl{In longer documents, we noticed an improvement in explicit reporting for details regarding the task interface (72\% for long, 35.7\% for short), instructions (66.4\% for long, 35.7\% for short), and the reward strategy (88.1\% for long, 60.7\% for short). The other attributes also show an increase, but the level of reporting is under 50\%.}

%               Attribute value.Y.E value.Y.I value.U value.N
% 13 Task interface source       4.1       1.2     0.0    94.7
% 14         Time allotted      38.0       5.9     1.2    56.1
% 15          Instructions      61.4      19.3     0.0    19.3
% 16        Task interface      66.1      17.5     0.0    16.4
% 17       Reward strategy      83.6       5.3     1.2    11.1
% 18             Task type     100.0       0.0     0.0     0.0


% Y.E long
% instructions 0.664
% reward 0.881
% interface 0.72

% Y.E short
% instructions 0.357
% reward 0.607
% interface 0.357



% quality control
\subsubsection*{\textbf{Quality control}} Quality control mechanisms can take place before, during, and after the task. Despite their importance, the papers did not fully report the mechanisms employed.
%
\hl{Most reported attributes include the criteria used to reject contributions (rejection criteria, 64.1\%), the mechanisms used after the task to safeguard quality (post-task checks, 55.6\%), and in-task mechanisms for quality control (in-task checks, 57.1\%). Though we found cases where these attributes were addressed rather implicitly (12.4\% for rejection criteria, 3.3\% for post-task checks, and 1.7\% for in-task checks)\footnote{\hl{Examples of implicit reporting of rejection criteria would be when one could infer a paper actually accepted all contributions and filtered out on the data analysis part based on a metric like completion time, or a participant was not considered because they did not provide some demographic information.}}}.
%
\hl{Training sessions, when applicable, were reported by only 34.1\% of the papers. And details regarding the redundancy employed (number of votes per item) and aggregation method were reported by 44.6\% and 35.2\% of papers, respectively. In cases where gold items where used as quality checks, only 29.2\% of papers reported explicitly the configuration (gold items configuration).}
%
Dropout prevention mechanisms, closely related to engagement, were reported by very few papers \hl{(7.1\%)}. 
%
As for the reporting style, quality control attributes are described as text, with few cases relying on additional tables and figures to report information such as the number of votes per item (1 paper) and training sessions (2 papers).
%
\hl{Although, for the most part, still inadequate, there is an increase in explicit reporting in 6/8 attributes for long papers, though only two of these are reported by at least 50\% of papers (rejection criteria 64.6\%, and in-task checks 57.6\%).}


%                         Attribute value.Y.E value.Y.I value.U value.N
% 17 Dropouts prevention mechanisms       7.1       3.0     1.2    89.9
% 18       Gold items configuration      29.2       3.5     0.0    67.3
% 19                       Training      34.1       1.4     0.0    64.5
% 20             Aggregation method      35.2       1.7     0.8    63.1
% 21       Number of votes per item      44.6       5.4     2.3    50.0
% 22                 In-task checks      57.1       1.7     0.0    41.2
% 23               Post-task checks      55.6       3.3     0.8    41.1
% 24             Rejection criteria      64.1      12.4     1.3    23.5










% outcome
\subsubsection*{\textbf{Outcome}} 
The number of participants is reported in most cases (by \hl{90.1\%} of the papers), and by inference, the number of contributions, described explicitly in just \hl{56.2\%} of papers.
%
\hl{In some cases, 5.8\% of papers for number of participants and 10\% for number of contributions,  these details were not explicitly addressed, and we coded as implicit (e.g., the number of participants could be inferred based on the total number of contributions and the contributions per annotator).}
%
Data processing steps on top of the contributions from the crowd are reported by \hl{61.5\%} of the papers.
%
For the rest of the attributes, the papers do not paint a clear picture. For example, only \hl{21.6\% to 31.6\%} of the papers reported explicitly discarded data and excluded participants (due to quality or rejection criteria), and just \hl{9.9\%} described dropouts (workers leaving the experiment for different reasons). 
%
The output dataset and participant demographics were also poorly reported, with only \hl{8.8\% and 34.7\%} of the papers providing these details explicitly.
% 
Papers reported the attributes mostly as text, accompanied by figures and tables for attributes such as the number of participants \hl{(21 papers) and contributions (11 papers)}, and participant demographics (5 papers).
%
\hl{For long documents, we noticed an increase in explicit reporting of 5/8 attributes, though, for the most part, reporting of these attributes is under 40\%, except for data processing (63.5\% for long, 50\% for short) and the number of contributions (57\% for long, 52.2\% for short)}.


%                   Attribute value.Y.E value.Y.I value.U value.N
% 17           Output dataset       8.8       2.9     0.0    88.3
% 18             Dropout rate       9.9       2.4     0.0    87.7
% 19           Discarded data      21.6       5.6     1.6    72.8
% 20    Excluded participants      31.6       1.9     1.3    66.5
% 21 Participant demographics      34.7       2.4     0.0    62.9
% 22          Data processing      61.5       1.5     0.0    37.0
% 23  Number of contributions      56.2      10.0     0.8    33.8
% 24   Number of participants      90.1       5.8     0.6     4.1








% requester
\subsubsection*{\textbf{Requester}} Overall, the attributes in this dimension were vastly under-reported.
The papers reported the most basic information, the selected platform, but they poorly addressed the rest of the attributes (\hl{6/7 attributes reported explicitly by 6.5\% to 22.9\% of the papers}).
%
Most of the under-reported attributes relate to the ethics of the experiment. These attributes cover if compensation was fair (at least a minimum wage), whether workers gave their consent and were aware they took part in an experiment, if the study received ethical approvals and were in compliance with data privacy policies.
%
Regarding the reporting style, the papers described these attributes as text.
%
\hl{Interestingly, we noticed an improvement in recent years from an ethical perspective, when comparing papers from \textit{2013-2016} and \textit{2017-2020}. Reporting ethical approvals, fair compensation, and privacy and data treatment attributes increased. This insight aligns with current works addressing issues such as underpayments in crowdsourcing (see \cite{DBLP:conf/chi/BarbosaC19} for a brief overview). However, these improvements in reporting are still far from ideal.}


%                       Attribute value.Y.E value.Y.I value.U value.N
% 15             Ethical approvals       7.6       1.8     0.0    90.6
% 16      Privacy & Data Treatment       6.5       3.0     0.0    90.5
% 17       Participation awareness       8.8       2.9     1.8    88.3
% 18              Informed consent      14.6       1.8     0.6    83.6
% 19 Requester-Worker interactions      18.2       0.6     0.0    81.2
% 20             Fair compensation      22.9       3.6     4.1    73.5
% 21              Platform(s) used      98.8       1.2     0.0     0.0








\subsection{Potential threats to validity}

The strength of the experimental evidence, as well as the ability of researchers to repeat and reproduce experiments, relies on the underlying methodology and how well this methodology and results are described. 
We have observed a reporting gap for the different dimensions in our taxonomy, which raises questions about experimental validity of crowdsourcing experiments reported in the literature. This section briefly discusses issues associated with under-reported attributes and how these connect to known biases from experimental research \cite{pannucci2010identifying} that affect the validity and integrity of scientific experiments.

% In the following, failed to report = Unclear + Not reported.

\subsubsection*{\textbf{Sampling bias}} Researchers can introduce bias by inferring conclusions from a sample that is not representative of their target population. In crowdsourcing this can happen by not properly defining (or reporting on) a target population or because the mechanisms provided by the platform (or implemented by the researchers) fail to obtain a proper sample.    
%
As observed, the concrete target population and sampling mechanisms were not properly reported by \hl{38\% and 84.2\%} of the papers, respectively. The resulting demographics were omitted for \hl{62.9\%} of the experiments -- without weighing in the mechanisms to derive this information.
%
Even returning workers, under-reported by \hl{68.7\%} of the papers, may also bias the sample since these can hinder the goal of reaching a broader and more diverse set of workers.
%
The lack of proper reporting of these attributes not only affects the proper assessment of population samples, but it may also introduce practical challenges to replicability given the diverse characteristics of crowd worker populations.  





\subsubsection*{\textbf{Selection bias}}
Bias can also occur due to the strategies chosen to assign participants to different conditions or cohorts. 
In crowdsourcing this could happen, for example, when the tasks associated to different conditions are executed under different operational settings (such as the ones mentioned in the following).    
%
Of the analyzed papers, \hl{83.6\%} did not report over what timeframe the experiment run, which is known to determine the characteristics of the active pool of workers \cite{DBLP:conf/wsdm/DifallahFI18}.
%
In this context, under-reporting how the conditions were executed, as in \hl{33.9\%} of the papers, can amplify this issue and render conditions with different sets of workers (e.g., conditions run sequentially with one capturing workers typically active during the morning and other conditions with night workers).
%
Task design attributes can also influence what type of workers are attracted to the tasks in the experiment. We observed \hl{19.3\%} of papers failing to report the instructions, \hl{12.3\%} the compensation, and \hl{57.3\%} the time constraints associated with the tasks. 
%
Reporting on these attributes is thus important, as they can reveal unintentional and intentional bias benefiting experimental conditions. 




\subsubsection*{\textbf{Observation and response bias}} 
Also called the ``The Hawthorne Effect" \cite{sedgwick2015understanding}, observation bias arises when participants, being aware that they are taking part to a study, modify their behavior or contributions.
%
In a crowdsourcing experiment, this might be triggered when providing informed consents and acknowledging the scientific purpose of the task or, as made clear by the experts, in a more subtle way by the requester name, task design and even by the (fair) compensation.
In relation to this, participants might feel compelled to orient their responses towards what they believe the expected findings are, in what is called response bias. 
% 
Only a few papers reported on participation awareness, and \hl{90.1\%} failed to report whether participants were informed of contributing to a study.




\subsubsection*{\textbf{Design bias}}
Researchers may fail to account for inherent biases present in experiments leading to what is called design bias. In crowdsourcing, in addition to other forms of experimental bias, there is a large body of literature on different forms of bias introduced by all aspects of task design and execution \cite{DBLP:conf/hcomp/WuQ17,DBLP:conf/www/HoSSV15,DBLP:conf/chi/SampathRI14,maddalena2016crowdsourcing,DBLP:journals/imwut/GadirajuCGD17,Qarout2019PlatformRelatedFI}. 
%
Our analysis shows that \hl{20.6\%} of the papers under-report how the experimental design was mapped to the selected crowdsourcing platform. 
%
Moreover, papers omitted information related to task design such as interface (\hl{16.4\%}), instructions (\hl{19.3\%}), and compensation (\hl{12.3\%}).
Even the implementation of desirable practices, such as running pilots to refine the experiments design, was reported explicitly in only \hl{27.5\%} of the papers.
This information gap can open the room to non-comparable conditions, especially when translating the experiment to other platforms with different features and workers.



\subsubsection*{\textbf{Measurement bias}} 
Bias can arise from measuring instruments of varying quality or errors in the data collection process. In crowdsourcing contexts, we can associate this bias to quality control. Overall, quality control attributes were under-reported, with \hl{41.9\%} of papers failing to report post-tasks checks, \hl{41.2\%} in-task checks, and \hl{64.5\%} did not describe training sessions.
%
Omitting these details may raise questions about the quality of the collected data, and allow for differences in quality when trying to rerun (or build upon) an experiment. For example, one could obtain better results by including training sessions.






\subsubsection*{\textbf{Ethical integrity}}
We observed that the vast majority of the papers failed to report on attributes such as fair compensation (\hl{77.6\%}), informed consent (\hl{84.2\%}), privacy \& data treatments (\hl{90.5\%}), and ethical approvals (\hl{90.6\%}). 
%
Not reporting on these attributes makes it difficult to assess whether experiments followed ethical guidelines and made sure workers were treated fairly and not exposed to any harm. This is clearly the ultimate goal. Understandably, processes for securing the ethics of experiments may vary from one institution to another, with some institutions enforcing ethical approvals on all studies while some put the burden on the researchers. What is clearly missing, and reflected on the interviews with experts and our own experience, are practical ethical guidelines that would allow researchers to make informed decisions about their crowdsourcing experiments, and proper support from crowdsourcing platforms to make sure these guidelines can be properly observed.

==> CSCW 2021 - Reporting crowd experiments/sections/taxonomy.tex <==
\section{Data \& Methods} \label{sec:methods}



Our goals in this work are to 
i) understand the status of reporting on crowdsourcing experiments to assess which aspects are covered or neglected and the extent to which reporting is consistent across the literature, and 
ii) provide guidelines for reporting to assist in achieving consistency in current practices and facilitate reproducibility and assessment.



% In doing so, we follow a systematic process comprising:
% \begin{enumerate}
%     \item \textbf{Identification of relevant crowdsourcing experiment attributes}. We start from understanding which design attributes are known to influence crowdsourcing experiments, and could potentially affect experiment outcomes and assessment, if misinterpreted, missing or under-reported. These attributes are captured in a taxonomy.
%     \item \textbf{Analysis of the state of reporting of crowdsourcing experiments}. We survey a sample of recent crowdsourcing experiments published in top venues, to get a picture of the current state of reporting, identify areas that need more support and highlight potential threats to validity. 
%     \item \textbf{Elaboration of reporting resources for crowdsourcing experiments}. We explore potential solutions and implementations for the reporting of crowdsourcing experiments, informed by the taxonomy of relevant design attributes and feedback from experts in the field. One promising reporting resource, a checklist, is further developed and validated.
% \end{enumerate}

% these three steps were informed from a mix of literature reviews and input from experts


To achieve these goals, we draw inspiration from standardizing efforts in evidence-based medicine and software engineering for the reporting of systematic literature reviews \cite{Prisma,Kitchenham2007}. We follow a mixed approach that involves (1) deriving a taxonomy of relevant attributes characterizing crowdsourcing experiments, (2) leveraging this taxonomy to analyze \hll{171} papers published in major venues and get a picture of the current state of reporting, and (3) exploring potential alternatives of guidelines for reporting. 


%\subsection*{Semi-structured interviews with crowdsourcing experts}
% {\color{royalblue(web)}
% crowdsourcing experts
% contacted through the extended network of the authors
% authors who have published in sigchi conferences and with a research track..
% authors who have performed experiment to study crowdsourcing (crowdsourcing main area of research), 
% used crowdsourcing to run user studies as well as experiments.

% 10 participants agree to participate (2F, 8M)
% August-September 2020


% The interview was organised in three parts that provide input to each of the three mains steps..
% trasncription and analysis

% Link to the protocol}





% \smallskip
%\noindent\textit{Expert interviews}. 
These steps were supported by  literature reviews and  interviews with experts in the field.
Specifically, literature reviews informed the first two steps, with a specific review for each step, and we describe them in detail in Sections \ref{sec:taxonomy} and \ref{sec:state}, respectively. 
The interviews with field experts provided a formative feedback along the entire process. They consisted of semi-structured interviews with researchers with
ample experience i) performing experiments to study crowdsourcing (i.e., crowdsourcing was the main area of research), or ii) leveraging crowdsourcing platforms to run user studies and experiments on different domains. Participants were recruited from the extended network of the authors, considering as eligibility criteria a research track involving crowdsourcing experiments and publishing in SIGCHI conferences.
%
\hl{Ten} experts agreed to participate (2F, 8M) including 1 Ph.D. student, 6 senior researchers from academia and industry, and 3 professors.


The interviews took place over Skype and Zoom between August and September 2020. Before the start of the sessions, participants were informed of the goal and scope the interview and provided their consent to participate and for the session to be recorded. The interview (see the protocol in Appendix \ref{sec:interview-protocol}) was organized into three parts that provided input to each of the three main steps in our methodology. The interviews were carried out independently by two researchers. All interviews were held in  and transcribed to English by the interviewer. Only the transcripts were accessed for the analyses. The analyses performed and how they inform our entire process are described in its proper context in the following sections. 

% {\color{royalblue(web)}
% ---- these goes within the following subsections
% part 1
% - what design choices are more critical and my affect experiment outcomes
% - what aspects were deemed relevant and should be reported
% - what aspects are under-reported or poorly reported

% part 2
% feedback on two of the six dimensions of crowdsourcing experiments that constitute the taxonomy
% - framing
% - completeness

% part 3
% - input and feedback on how appropriate reporting resources
% two options were brought up
% - offloading
% - checklist
% ---
% }



















\section{A taxonomy of relevant attributes for crowdsourcing experiments} \label{sec:taxonomy}

This section introduces the taxonomy of relevant attributes that characterize different aspects of crowdsourcing experiments.
%
The attributes are grouped around six main dimensions denoting: the task requester, the experimental design used, the participants of the experiments (i.e., the crowd), the task design and configuration, the quality control mechanisms used to guard the quality of the results, and the outcome of the experiment.
%
% \hl{
% Notice, however, that our aim is on the comprehensiveness in terms of the attributes we identified and not the way we organized these into dimensions, which is a specific way of viewing things. For example, the demographics attribute in Outcome could be thought of as part of the Crowd dimension, but the semantic behind this attribute is whether the results also include demographic information, while the Crowd dimension refers to the criteria used to filter and select workers\footnote{\hl{One could indeed use demographics to select workers but ultimately do not report these in the experiment results.}}.
% }
% %
The resulting taxonomy is summarized in Figure \ref{fig:taxonomy}. In the following we describe the methods and described in detail the final taxonomy, highlighting the literature support and expert opinions. 





\input{sections/methods-taxonomy}







\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{figures/taxonomy.pdf}
  \caption{A taxonomy of relevant attributes characterizing experiments in crowdsourcing.}
  \Description{A taxonomy of relevant attributes characterizing experiments in crowdsourcing.}
  \label{fig:taxonomy}
\end{figure}






\subsection{Experimental Design}



The experimental design represents the building block for experiments of any kind, allowing to set the tone of the study and what level of conclusions can be derived from the experimental results.
%
Proper experimental research involves several elements, from the research questions to the study design and analysis.
%
These are well-understood aspects covered in experimental research guidelines and textbooks on research methods (e.g., \cite{Gergle2014, OlsonKnowingHCI}). %and tend to be communicated effectively in the research methods section of scientific publications.

The \textit{experimental design} section of the taxonomy we propose focuses instead on those attributes that are more closely related to crowdsourcing, and that allow experiments to be run in such platforms.
%
%The \ding{108} \textit{input dataset} fuels the task workers solve and is therefore crucial that authors communicate how this dataset was obtained and whether it is publicly available.
%
The limited support for running experiments in crowdsourcing platforms translates into many alternative strategies to map the experimental design to crowdsourcing tasks. %, making a simple between-subjects design a challenge  \cite{DBLP:conf/chi/KitturCS08}. 
Having multiple alternatives (and failing to accurately report these) can introduce confounds and ultimately affect the reproducibility of crowdsourcing experiments \cite{Qarout2019PlatformRelatedFI}. 
%
%The \ding{108} \textit{experimental design to task mapping} attribute indicates first what study design was used and, second, how the experimental conditions were mapped to crowdsourcing tasks. 
The \ding{108} \textit{experimental design to task mapping} attribute indicates how the experimental conditions (e.g., Condition A and Condition B) were mapped to crowdsourcing tasks. 
%For example, the experiment could use a between-subjects design and map each condition as a micro-task in a crowdsourcing platform.
For example, as shown in Figure \ref{fig:experiment-mapping}, a between-subjects design could map each experimental condition to a different micro-task (Condition A $\rightarrow$ Task~2, Condition B  $\rightarrow$ Task~1) or randomize them within a single task (Conditions A,B  $\rightarrow$ Task 1).
%
Followed by this design choice, it is also relevant to define whether the experimental conditions were executed in parallel or sequentially (i.e., the \ding{108} \textit{execution of experimental conditions} entry in the taxonomy) as different execution strategies may result in experimental conditions leveraging different sets of active crowd workers (e.g., population samples with different underlying characteristics). 



Another factor comprises participant's \ding{108} \textit{allocation to experimental conditions}. %True experiments require random assignments of participants to conditions
%The strength of the resulting experimental evidence is affected by if and how the randomization of the assignments was performed.
This attribute captures \textit{if} and also \textit{how} the randomization of the assignments was performed, considering the effect on the strength of the resulting experimental evidence. %; therefore, studies must report \textit{if} and also \textit{how} this was achieved.
%
In crowdsourcing environments, where multiple micro-tasks may be running in parallel or sequentially to serve the overall experimental design, crowd workers may be able to engage in more than one micro-task, leading to what we refer to as \ding{108} \textit{returning workers}. 
Depending on the experimental design and how it was handled, this situation may be desirable or introduce unintended biases affecting the integrity of the experimental conditions and, ultimately, the experiment results \cite{Paolacci2010RunningEO,CrowdHub2019}.
%This situation can result in unintended biases affecting the comparison of experimental conditions and, ultimately, the experiment results \cite{Paolacci2010RunningEO,CrowdHub2019}. %Therefore, crowdsourcing experiments need to account for and communicate how returning workers were dealt with (or prevented in the first place).
Therefore, this entry in the taxonomy captures whether crowdsourcing experiments account for and communicate how returning workers were dealt with (or prevented in the first place).



The global scale of crowdsourcing platforms makes the active pool of workers to vary throughout the day \cite{DBLP:conf/wsdm/DifallahFI18}. Thus, failing to account for (and therefore report on) this aspect may add confounding factors to the experiment that hurt its reproducibility \cite{Qarout2019PlatformRelatedFI}. The taxonomy, therefore, needs to capture the \ding{108} \textit{\hl{execution timeframe}} of the experiment, by answering the simple question: over what timeframe was the experiment executed? (e.g., the experiment ran between January 1 and 10, every day at 2 PM).
%
The \ding{108} \textit{input dataset} fuels the task workers solve and is therefore crucial to indicate how this dataset was obtained and whether it is publicly available.
%
Lastly, the crowdsourcing literature advises to fine-tune a crowdsourcing experiment through multiple pilots \cite{DBLP:journals/jmlr/Vaughan17,DBLP:journals/sigkdd/MasonW09}, and it is intuitively relevant that authors report whether \ding{108} \textit{pilots} were performed before the main study.




%\smallskip
%\noindent\textbf{Expert opinion}.
\subsubsection*{\textbf{Expert opinion}} 
The interviews with experts organically touched on several of the experimental design attributes of crowdsourcing experiments, and while no new attributes emerged, their input allowed us to better scope and articulate the attributes. Their comments also provide a window into the challenges faced by experts in porting (and reporting on) experimental designs into crowdsourcing platforms.

Experts highlighted the importance of the experimental design in crowdsourcing experiments, indicating that ``\textit{the design is very critical}'', and at the same time acknowledging the challenges posed by the uncontrolled environment provided by crowdsourcing platforms. One participant illustrated this aspect while bringing up the importance of the allocation of crowd workers to experimental conditions
\begin{quote}
\textit{    ``In the ideal case, if you [had] a full control of the crowdsourcing platform, you would actually be able to do [a proper] randomization of crowd workers [to experimental conditions]. And being a requestor in a crowdsourcing platform such as AMT or Crowdflower, you don’t have this opportunity (...) Therefore, by not having these opportunities you kind of [perform] certain workarounds.''}
\end{quote}

%%%% Allocation to experimental conditions
% We do not have a control of a crowdsourcing platform. In the ideal case, if you would have a full control of the crowdsourcing platform, you would be actually be able to do the randomisation of crowd workers for example. And being a requestor in a crowdsourcing platform such as AMT or Crowdflower, you don’t have this opportunity to do nice randomisation. 
% Therefore, you by not having these opportunities you kind of do certain workarounds which create certain bias. 

The importance of experimental design to task mapping, execution dates, execution of experimental conditions and returning workers were all covered by the participants during the interview. One expert conveyed through an illustrative example how all these aspect are interconnected:

\begin{quote}
\textit{    Let's say you have two [conditions], like in an A/B test, and what differs in the two [associated] tasks is a design, literally a UI design. Then what you do is you run one task at 1pm today, and the other task tomorrow at 1pm as well. Well, time of the day is kind the same, but at the same time tomorrow [the platform would have a] slightly different population than today. It is very hard to control for some things. Maybe some participants that participate in your task today, will participate in your task tomorrow (recurrent workers), which definitely creates a certain bias and a ``feel of work" effect.} 
\end{quote}

Accessing input dataset and other more general aspects of experimental design not covered by the taxonomy (e.g., hypotheses, research questions) were also mentioned. One participant went as far as to say that even in ideal case where all information is available, even running the experiment under a different requester name could introduce bias \textit{``your requester name might be NASA (..) and people are just so excited to participate in studies run by NASA. It doesn’t mean that the effect is huge, but we know it [introduces] bias''. }

%%%% Experimental design to task mapping
%%%% Execution date
%let’s say you have two versions, like an A/B test, and maybe what differs in these two tasks is a design, literally a UI design. Then what you do is you run one task at 1pm today, and then you decide, ah, let me run another task tomorrow at 1pm as well. Well, time of the day is kind the same, but at the same time tomorrow [would have a] slightly different population than today. It is very hard to control for some things. Maybe some participants that participate in your task today, will participate in your task tomorrow, which definitely creates a certain bias and a “feel of work” effect. 

%%%% Some participants went further to highlight how even in similar situation the smallest differences can introduce counfounds
%So this will allow me to repeat the exact same experiment, but with a different requestor name. Even this is already a difference, you may have a female name, your requestor name might be NASA. You may remember these studies that people are just so excited to participate in studies run by NASA. This all affects, it doesn’t mean that the effect is huge, but we know it create certain bias. 




% %para summarizing feedback for Exp design
% The design of the study is essential to the experiment, as explicitly indicated by one of the participants (e.g., ``\textit{I would say, the design is very critical for the whole thing}'').
% %
% Participants (\textbf{\color{red}N=4}) deemed relevant aspects such as the study design, hypotheses, strategies used to avoid biases (e.g., randomization), and assignment of subjects to conditions.
% %
% As for poorly-reported aspects, participants (\textbf{\color{red}N=4}) indicated that it is difficult to access the input dataset used in the experiments they are interested in. Or they have a hard time understanding the exact steps to prepare this dataset for the experiment due to missing details in the papers.
% %
% One of the participants indicated that reviewers tend to ask for the input dataset. However, there are situations where privacy regulations may prevent its publication: \textit{``Because of the raw data we use, we can not publicly expose it. We usually just describe it, which could make people ask how the actual raw dataset looks like.''}.















% Explain, why is relevant.
% encompases many attributes that are required to reproduce and analyse an experiment - research methods.
% focus of guidelines.

% In relation to crowdsourcing..

% Input dataset

% how you do the mapping, many approahces that can introuce counfunoundig variables -- many alternatives.
% Experimental Design to task mapping
% Execution of experimental conditions
% \textit{Assignments to experimental conditions}


%Execution dates
%Pilots
%Returning workers


% basic components of experimentations
%     research question / hypothesis
%     variables (independent, dependent, control, covariates)
%     participants (and their characteristics, e.g., demographics)
%     experimental conditions
%     random assignments
    
% research design
%     randomized experiments (between-subjects design, within-subjects design, factorial designs, mixed factorial designs)
%     sample size
%     quasi-experiments (Non-equivalent Groups Design, Interrupted Time-Series Design)



\subsection{Crowd}

The active pool of workers in crowdsourcing platforms constitutes the population of human subjects who can participate in crowdsourcing experiments.
% - crowdsourcing allows to reach participants at scales that too difficult and cost in laboratory settings, which appeals researchers [cite probably Mason09 or Kittur]
% - the population in one platform may differ from the one found in a different crowdsourcing platform [Qarout2019PlatformRelatedFI]
% it provides means to scale up previously laboratory experiments which tend to resort to a small pool of subjects [] 
%
The \ding{108} \textit{target population} aims to explicitly capture the eligibility criteria used to screen crowd workers and determine potential participants of the experiment. Conversely, this entry captures if no specific criteria were applied, thus implicitly using the characteristics of workers in the selected crowdsourcing platform as eligibility criteria (i.e., the entire crowdsourcing population is considered eligible). 
%
For example, studies may consider using specific demographic attributes, concrete environments in which workers perform their work (OS, web browser, mobile phones), a threshold to the task acceptance rate, or the number of tasks completed (typically provided by the platforms).
% some sentences to say why this is important


Once the target population is defined, the \ding{108} \textit{sampling mechanism} describes what strategies were used to recruit a diverse or representative set of participants from the target population.
%
Crowdsourcing environments give researchers more affordable access to a large and diverse pool of subjects with a wide range of demographic attributes, as opposed to laboratory settings where scale (and diversity) is constrained by time and available funds \cite{RAND2012ThePromiseOfAMT,DBLP:conf/dagstuhl/GadirajuMNSEAF15}.
%
This diversity plays an essential part in the external validity of an experiment, similarly to how the soundness of the methodology contributes to its internal validity (indeed, crowdsourcing experiments can be both internally and externally valid as their laboratory counterparts \cite{Horton2011}).
%
However, sampling strategies in crowdsourcing environments face additional challenges not found in traditional settings. For example, how the underlying demographics are in flux based on the active workers \cite{DBLP:conf/wsdm/DifallahFI18}; the lack of control over the subjects \cite{DBLP:conf/dagstuhl/GadirajuMNSEAF15}; and how easy it is for workers to quit, potentially causing non-random attrition and rendering the experimental conditions unbalanced \cite{RAND2012ThePromiseOfAMT}.




\subsubsection*{\textbf{Expert opinion}} 
The interviews with the experts addressed and enriched the two attributes associated to this dimension. 
Participants also emphasized how crucial (and challenging) it is to find the right workers who suit the needs of the study and can participate in it, and make sure a reasonable and representative sample is obtained from this target population.

Accordingly, both the worker profile making up the target population and the mechanisms used to sample participants were deemed relevant by participants, giving examples such as demographics (\textit{``I think is important to get to know some properties of the workers''}) and screening and qualification strategies applied to workers (\textit{``First is your recruiting requirement that includes the screening process: how you selected your participants, you need to describe that''}). 

Some participants went as far as to suggest that the mechanisms for inferring the properties of the target population, such as demographics and qualifications, are important and should be reported. For example, 

% Speaking about population, you can be very strict I think. We are coming back to, some tasks are designed in a so academic way, you are literally being asked “what do you see in the picture” and you maybe need to transcribe the picture, and then you have 25 questions about you age, income, race and something like that. I am a bit skeptical about this task design because first of all, it creates a huge bias. You know, it’s an academic study, you might really enjoy faking it, you hate certain parts of the population, and you could just choose that part of the population and produce irrelevant results for example

% It might depend on different platforms, in some platforms you might get some data about the population."        
        
\begin{quote}
\textit{``Some tasks are designed in a so academic way. You are literally being asked `what do you see in the picture' [prompting the worker to annotate the picture], and then you have 25 questions about your age, income, race and something like that. I am a bit skeptical about this task design because first of all, it creates a huge bias. You know it's an academic study, you might really enjoy faking it, (..) or produce irrelevant results for example.
It might depend on [the] platform, in some you might get some data about the population.''}
\end{quote}

In relation to the above, another participant reflected on some uncertainties about using demographics, casting some light into the above behavior \textit{ ``it's not always clear if the gender of the participants is expected to be collected and reported, since not always [it] is relevant but it might be required by the reviewers''}.

The participants also provided specific examples of sampling strategies used in their experience, including sampling over time and geographical regions. 


% Participants (\textbf{\color{red}N=5}) emphasized how crucial (and challenging) it is to find the right workers who suit the needs of the study and can participate in it, and make sure a reasonable and representative sample is obtained from this target population.
% %
% Likewise, both the target worker profile and the mechanisms used to sample participants were deemed relevant by participants (\textbf{\color{red}N=7}), giving examples such as demographics (\textit{``I think is important to get to know some properties of the workers''}) and filtering conditions applied to workers (\textit{``First is your recruiting requirement that includes the screening process: how you selected your participants, you need to describe that''}).
% %
% One participant mentioned that papers indicate they make sure the population was diverse, avoiding demographic biases, but failing to report how this was achieved.






\subsection{Task}

The actual crowdsourcing tasks solved by workers can be regarded as the actual instruments or materials presented to the participants. The group of attributes presented here characterizes the tasks delivered as part of crowdsourcing experiments, considering organizational and operational details known to affect the results.


The nature and goal of the experiment shape the kind of tasks that are sent down to workers in crowdsourcing platforms, these aspects have been considered by previous research to propose a categorization of micro-tasks \cite{DBLP:conf/ht/GadirajuKD14}; we included in the taxonomy the \ding{108} \textit{task type} attribute to capture this information.

The \ding{108} \textit{task interface} in tandem with the \ding{108} \textit{instructions} concern the exact user interface and guidelines presented to workers. Poorly written instructions can misdirect workers and affect their performance in the experiments, resulting in subpar responses \cite{DBLP:conf/hcomp/WuQ17}. Besides, it can also reduce task intake and negatively affect how long the experiment takes to finish \cite{DBLP:conf/wsdm/HanRGSCMD19}. 
%
Variants of a task interface could unravel performance differences \cite{Mortensen2016crowd}. And similarly, current evidence suggests enriched interfaces may aid workers, allowing them to attain higher performance \cite{DBLP:conf/chi/SampathRI14,Wilson2016WWW,ramirez2019}.
% 
The full disclosure of operational details such as task and instructions materials favors reproducible research. To this end, the taxonomy also captures the exact \ding{108} \textit{task interface source} (typically a combination of HTML, CSS, and JavaScript) uploaded to the crowdsourcing platform or related system (e.g., TurkServer \cite{DBLP:conf/hcomp/MaoCGPPZ12}).




The \ding{108} \textit{time allotted} workers to perform the task, as well as the \ding{108} \textit{reward strategy} used to motivate them, can also influence the progress of the experiment and resulting performance of workers.
%
In general, extrinsic factors such as proper monetary rewards can impact how much workers contribute \cite{Mason2012}. For effort-intensive tasks, in particular, adequate payments can motivate workers to produce results of higher quality \cite{DBLP:conf/www/HoSSV15}.
%
Low payments, however, may curb task intake and affect how fast experiments progress \cite{DBLP:conf/icwsm/RogstadiusKKSLV11,DBLP:conf/wsdm/HanRGSCMD19}.
%
Payment mechanisms are not limited to the amount being paid but also how. Different payment strategies could also lead to effects on how workers perform \cite{difallah2014scaling}.
%
Tasks can also include elements that target intrinsic motivational factors, for example, to aid how workers engage and commit \cite{DBLP:conf/lak/GadirajuD17} (although one could argue that intrinsic factors are effects we may want to reduce in an experimental setting unless it is the subject of study).
%Crowdsourcing can also resort to intrinsic factors to motivate workers; examples of this are games with a purpose \cite{DBLP:journals/computer/Ahn06} and the Galaxy Zoo project \cite{GalaxyZoo} (though one could argue that intrinsic enjoyment may not transfer well among different tasks).
%
The time allotted workers to spend on the task naturally limits the associated cost of the experiment, besides studies in cost-effective crowdsourcing shed light on the impact of time on worker behavior and performance \cite{maddalena2016crowdsourcing,krishna2016embracing}.
%
We draw on these reasons to include in the taxonomy attributes that capture what mechanisms were employed to reward and motivate workers and whether time constraints where imposed.



\subsubsection*{\textbf{Expert opinion}} 
Aspects of task design such as the clarity of the instructions, the task interface and compensation were all suggested as critical design choices for the success of crowdsourcing experiments. Intuitively, participants  indicated that these aspects are relevant and must be reported.

Participants weighted in regarding different levels of information provided about the task interface, some mentioning that, for example, the reporting of the task interface should go beyond screenshots to include links to source files (\textit{``people report task design like a screenshot [...] It is maybe relevant to report the actual task design, like HTML, JavaScript, CSS files, so that people can reproduce it''}). Other experts, provided more nuanced opinions, e.g., 
\textit{``If there is a paper that talks about different treatments that are interface-related and there is no interface, it is a red flag. If there is no source code, it’s a yellow flag - for me at least.''}

In relation to the above, instructions and task descriptions were deemed critical. One participant illustrated how this information could completely shape the outcomes of an experiment, in the specific case of open-ended input: 
\begin{quote}
\textit{  ``The prompts and tips that we are giving before starting the task will definitely impact the final result. So, for example, if you give any useful examples of the feedback that crowd workers can generate, most probably, all of the workers will start imitating the same examples.'' } 
\end{quote}


Instructions, along with the payment and perceived effort (time) affect were reported as influencing not only the quality of the results but the decision to participate in the first place.


% Aspects of task design such as the clarity of the instructions, the task interface, the complexity and granularity of the task, compensation, and priming were suggested as critical design choices for the success of crowdsourcing experiments (\textbf{\color{red}N=7}).
% %
% Intuitively, participants (\textbf{\color{red}N=8}) indicated that these aspects are relevant and must be reported, mentioning that, for example, the reporting of the task interface should go beyond screenshots and include a link where the source files are available (\textit{``people report task design like a screenshot [...] It is maybe relevant to report the actual task design, like HTML, JavaScript, CSS files, so that people can reproduce it''}).
% %
% Indeed, the task design and interface tend to be poorly-reported: \textit{``Usually people would say `this is the task and this is the result', we do not know what the crowd workers saw''}. 
% %
% Also, three participants indicated that how much workers are paid and task interface are not always clear in the papers they read. In situations where they missed this information in their papers, reviewers asked for clarifications (\textit{``reviewers sometimes ask for some screenshots of the interface [...] some reviewers asked about the payment, or they wanted more detail about the total amount''}).
% %
% One participant indicated that these details tend to be missed by papers where crowdsourcing is not the primary research focus, but rather used as a tool. However, we show in Section \ref{sec:state} that papers, where crowdsourcing is the subject of study, miss to report relevant aspects of the experiments.









\subsection{Quality Control}

The varying skills, motivations, backgrounds, and behavior of online workers make quality control a major challenge in crowdsourcing \cite{DBLP:journals/csur/DanielKCBA18}. Therefore, quality control mechanisms are fundamental to any crowdsourcing task to safeguard the resulting quality of the contributions. 
%
An initial step concerning quality is to define what constitutes an invalid answer or contribution, and the \ding{108}~\textit{rejection criteria} aims to capture this information.  

%- rejection criteria: What criteria were used to accept or reject a contribution from the crowd?
% mention something that comes from the paper on "framing task meaningfully"

Quality mechanisms can be set at different points in the crowdsourcing task. \ding{108} \textit{Training} protocols can be used to prepare workers for the job, which can have a positive impact on their resulting performance \cite{DBLP:conf/naacl/LiuSBLLW16}.
%
Another group of mechanisms can be categorized as \ding{108} \textit{in-task checks} or strategies embedded in the task to safeguard quality as contributions are collected. Whenever the nature of the task allows it, a fairly common practice is to embed gold items or attention checks to monitor the collected answers against the ground truth regularly. This simple technique can help to deal with malicious workers and avoid wasting collected contributions \cite{DBLP:conf/chi/KitturCS08}. 
%
The \ding{108} \textit{gold items configuration} attribute then captures how these items were selected (typically a subset of the input dataset), how frequently these gold items appear in the task, and what threshold was used to filter out workers underperforming on these items.
%
Other strategies involve imposing quality by design, such as adding feedback loops (where workers self-assess or receive external feedback) \cite{DBLP:conf/cscw/DowKKH12}, or making workers collaborate \cite{drapeau2016microtalk,schaekermann2018resolvable,Cicero2018}.



Another set of approaches are \ding{108} \textit{post-task checks} or mechanisms leveraged upon task completion, which can complement in-task checks and training protocols. 
%
Manual inspection (e.g., by an expert) can be used to review contributions from workers, limited by the scale of crowdsourcing and the cost associated with expert feedback \cite{DBLP:conf/cscw/DowKKH12}.
%
The assessment can also be computation-drive, for example, removing contributions that do not fall above a minimum time or agreement threshold \cite{DBLP:conf/websci/MarshallS13,DBLP:conf/cscw/HansenSCRG13}.

%
Depending on the type of task in the experiment, one may rely on redundancy, considering the \ding{108} \textit{number of votes per item} to be more than one, and leverage the same task to multiple workers to compensate potential noise. 
%
The \ding{108} \textit{aggregation method} comes in tandem with redundancy. A typical strategy is to use majority voting; however, more sophisticated and effective alternatives have been developed to derive the right answer even when the majority may be wrong (e.g., \cite{DawidSkene_Confusion,whitehill2009whose,Dong2013}).






Participants may drop out of experiments for different reasons and at different rates depending on the experimental conditions, introducing potential selection and attrition bias.
%
Different experimental treatments may be less appealing to workers and therefore result in non-random or selective attrition, introducing confounds in the experiment affecting the comparisons of the conditions \cite{Horton2011,RAND2012ThePromiseOfAMT}.
%
Copying with attrition, especially in online experiments, is instrumental to the study's internal validity, making sure dropouts stay roughly the same across conditions.
%
Therefore, the taxonomy captures what \ding{108} \textit{dropouts prevention mechanisms} were used to deal with the prevalence of task abandonment in crowdsourcing \cite{DBLP:conf/wsdm/HanRGSCMD19,kobren2015getting}.
%
For example, on Amazon Mechanical Turk, one can resort to using (neutral) qualification tasks to create a pool of potential participants and then send invitations to the actual tasks based on the assigned conditions \cite{DBLP:conf/www/HoSSV15}. 
%
Or, if one treatment incurs different effort levels than another, one may manipulate both treatments to include an effort-intensive activity and align how the difficulty of both tasks are perceived, regularizing the attrition rates \cite{RAND2012ThePromiseOfAMT}.





\subsubsection*{\textbf{Expert opinion}} 

Quality control was a hot topic during the interviews, cited as  \textit{``one of the biggest concerns in designing the tasks''}.
%
Participants considered quality control mechanisms as critical design choices that impact the results of experiments.  %Their input painted a clearer picture about the relevance of certain quality control attributes depending on the type of task. 
%

The quality control mechanism suggested by the participants focused on the task flow, from strategies applied before (e.g., training or qualification assessment), during (e.g., gold items and attention checks) and after the completion of the task (e.g., filtering out contributions). In describing the control mechanisms applied to specific experimental settings, the participants highlighted that quality control mechanisms and when they are applied depend on the type of task. 
%
In some contexts, involving open-ended tasks such as content-creation, strategies such as gold items may not be applicable, requiring manual checks after task completion. 
\begin{quote}
    \textit{ ``In my experiments, the main problem - and that you would always have - is that there is no golden data for the answers that the crowd workers provide. When we are asking the crowd workers to provide open-ended text or feedback or anything, they can write anything they like. Here the quality control is very challenging and almost near to impossible to achieve.''}
\end{quote}

Indeed, a participant cited the exploration of automatic approaches as a \textit{``major area of research''} in his/her domain. 

%The mechanisms suggested by participants can be grouped based on when they occur: either before (\textit{``I want this task to be done by Italian or US people''}, or \textit{``The prompts given to the crowd workers before starting the task''}), during (\textit{``the attention check varies depending on the study''}), or after the tasks (\textit{``we do like questionnaire at the beginning and then we use that to filter out afterward''}).





%Quality control in crowdsourcing is \textit{``[...] one of the biggest concerns in designing the tasks''}, mentioned P9.
%
%Participants (\textbf{\color{red}N=6}) considered quality control mechanisms as critical design choices that impact the results of experiments.
%
%The mechanisms suggested by participants can be grouped based on when they occur: either before (\textit{``I want this task to be done by Italian or US people''}, or \textit{``The prompts given to the crowd workers before starting the task''}), during (\textit{``the attention check varies depending on the study''}), or after the tasks (\textit{``we do like questionnaire at the beginning and then we use that to filter out afterward''}).
%
%In some contexts, like open-ended tasks, strategies such as gold items may not be applicable since \textit{``there is no golden data for the answers crowd workers provide''}.
%
%As such, aspects of quality control were deemed relevant and crucial to report in papers (\textbf{\color{red}N=5}). 
%
%However, detailed reporting of quality control aspects is not a frequent practice followed by paper authors, as mentioned by one participant, aligning with what we present in Section \ref{sec:state}.










\subsection{Outcome}


% Similarly to what we discussed in the experimental design, these are well-undertood aspects covered in guidelines for experimental research [APA cite]

% The statistical analysis of the results allows to test the hypothesese and answer the research questions governing the experiment.
% Existing guidelines offer support about what statistical methods to apply depending on the design and nature of the experiment. Similar to the experimental design dimension of the taxonomy, the outcome concerns about the details more closer to crowdsourcing.





The outcome dimension concerns details of the experimental results, more closely related to crowdsourcing, to aid their understanding, verification, and reproducibility.
%
The soundness of the data analysis process and how to articulate the findings aid to derive the right conclusions from experiments \cite{Gergle2014}. However, capturing these aspects are well beyond the scope of the taxonomy and refer them to available guidelines (e.g., \cite{StatisticsPrincipled1995,APA6thEDITION}).


The \ding{108} \textit{number of participants} and the \ding{108} \textit{number of contributions} collected (in total and across conditions) help to understand the scale of the experiment.
%
Also, the \ding{108} \textit{dropout rate} and \ding{108} \textit{demographics} quantify the level of attrition and diversity present in the experimental treatments, respectively.
%
Based on the rejection criteria, the experimenter may regard some of the contributions as invalid. The taxonomy identifies two related elements, the number of \ding{108} \textit{excluded participants}, perhaps malicious (or underperforming) workers, rendering a whole batch of answers from them as invalid. And \ding{108} \textit{discarded data}, i.e., specific contributions that were excluded before the data analysis.


While the previous attributes cover different quantities in the outcome, the \ding{108} \textit{data processing} captures any data manipulation step performed on the collected data. Intuitively, this information foster reproducible research alongside providing the \ding{108} \textit{output dataset} derived from the experiment (i.e., the raw or aggregated contributions from crowd workers).






\subsubsection*{\textbf{Expert opinion}} 
Interestingly, the comments from the participants would naturally flow more towards attributes that would allow researchers to repeat crowdsourcing experiments, and to a lesser extent the assessment of the outcomes.  
%
Among the few to touch on outcome attributes, two participants mentioned that the output dataset, as well as potential confounds like demographics, are relevant aspects of crowdsourcing experiments that should be reported (\textit{``it is important to report those aspects you did not control, such as demographic information''}).
%
%Despite their importance, participants mentioned that these details tend to go under-reported in papers (\textit{``I have not seen any paper specifying which country participated in the study'', or ``many papers just report datasets with votes already aggregated; not the individual crowd votes''}).








\subsection{Requester}

The task requester is the person (or group of people) responsible for the design and execution of the experiment.
%
The organizational and operational details related to how the requester set up the experiment are also important.
%
The selected crowdsourcing \ding{108} \textit{platform(s)} constitutes the environment in which the experiment runs. It represents an essential element that guides how the requester operationalizes the study based on the features offered by the platform.
%
However, the available functionality tend to be limited for the requirements imposed by the experimental design \cite{DBLP:conf/chi/KitturCS08}, often requiring requesters to implement additional features to cover this lack of support. 
%
These \ding{108} \textit{implemented features} represent additional experimental instruments that also affect how feasible it is to replicate an experiment.


This limited support also translates into the available tools to facilitate interactions with workers (e.g., chat rooms and emails). 
%
\ding{108} \textit{Requester-worker interactions} could potentially impact how workers engage and perform in the tasks from the experiment \cite{DBLP:conf/cscw/DowKKH12}, so it is important to capture in the taxonomy if and how these interactions happen.
%
However, simple designs may not require complex interactions (or no interaction at all). 
%
For example, requesters may not need to interact with workers to study task design in the context of classification tasks, relying entirely on leveraging clear guidelines to articulate what they expect from workers \cite{ramirez2019,Mortensen2016crowd}.






Crowdsourcing environments define new legal grounds where policies may not be sufficiently defined (see \cite{felstiner2011working} for a review of the legal aspects around crowdsourcing).
%
The community is increasingly voicing the need for \ding{108} \textit{ethical approvals} for experiments run in crowdsourcing environments \cite{GraberIRB2013,DBLP:conf/cscw/MartinHOG14}.
%
\ding{108} \textit{Informed consent} tends to be often required for research with human subjects, as well as \ding{108} \textit{privacy and data treatment} statements for experiments that need to collect and store sensitive information.
%
\ding{108} \textit{Fair compensation} is also a relevant aspect from an ethical perspective. \hl{Computing fair wages indeed represents an active research area, considering that providing a minimum wage is not necessarily fair \cite{Whiting2019FairWC}.}
%
Initially, crowdsourcing platforms such as Amazon Mechanical Turk were deemed a ``marked for lemons'' \cite{IpeirotisLemons2010}, an environment restraining committed workers from earning at least a legal minimum wage due to the prevalence of less-committed or malicious workers.
%
Proper compensation can become a more frequent practice due to current features (like qualifications or badges) in crowdsourcing environments, advances in techniques to safeguard quality, plus underpayment issues being a reiterating topic addressed by recent literature \cite{DBLP:conf/cscw/KitturNBGSZLH13,DBLP:conf/chi/HaraAMSCB18,DBLP:conf/chi/BarbosaC19,Whiting2019FairWC}.
%
Additional context can be given to online workers, so they become aware they take part in an experiment. 
%
This \ding{108} \textit{participation awareness} is a relevant aspect because it is known to play a role in participant behavior \cite{McCambridge2012Awareness}.







\subsubsection*{\textbf{Expert opinion}} 
%The relevant aspects suggested by the participants (\textbf{\color{red}N=3}) relate to the ethics of the experiment or the platform-specific features of the selected crowdsourcing platform.
%
The operational context navigated by the requester was prompted by the participants in terms of the treatment of crowd workers, data management, and the technical environment. 

%The ethics of the experiments or the platform-specific features of the selected crowdsourcing platform were deemed relevant by the participants. %(\textbf{\color{red}N=3}).
%
In terms of ethics and data management, participant stressed that workers should receive a fair compensation for their contributions and protected from potential harm, and that it should be clear that this is the case (\textit{``from the ethical perspective, [it should be reported] how much [crowd workers] were paid, whether they were exposed to certain content they were not naturally expected to see, like watching porn, cut bodies, and so on''}). Reflecting on the role of the different stakeholders in ensuring these practices, and whether ethical approvals should be required, some participant turned to practical recommendations:

\begin{quote}
    \textit{``I think [ethical] approval is a different thing. It is up to the institution where the researchers are from, but on the very generic case we just want to make sure that the crowd workers were told in advance [what they were exposed to]''}.
\end{quote}


%Workers should receive a fair compensation for their contributions, which could play a role in the quality of the results (\textit{``On the one hand, is fairness and, on the other hand, is the big impact it has on the quality of the output. If you do not pay well, then you could expect [...] low-quality output''}).
%
The friction between observing the privacy of the crowd workers while making sure enough data was collected was also raised \textit{``I think is important to get to know some properties of the workers. But of course, it has implications in privacy''}.
%As mentioned previously, it is important to know some characteristics of the workers, however, this has privacy implications (\textit{``I think is important to get to know some properties of the workers. But of course, it has implications in privacy.''}).

As for the technical environment, participants expressed the importance of reporting from simple attributes, such as the actual crowdsourcing platform, to platform-specific features and complex configurations. One participant illustrated the latter for quality control configurations (\textit{``the whole quality control mechanism has a set of parameters that you have to set up, complex parameters that can lead to complex settings''}). But even for platform, it was argued that the role should be properly described (\textit{``You can say that F8/Append is kind of a hub for accessing other different platforms''}). 
%
Moreover, the case of F8 (now Append) serving as a hub to other platforms could be problematic if it is not reported properly, as indicated by the participant: 
\begin{quote}
    \textit{``Very few papers tell you, I ran my stuff on F8, but under the hood, F8 was forwarding the tasks to these 50 different platforms [...] These are like variables you add to your experiment and make the whole thing so complex''}.
\end{quote}


% from the ethical perspective, how much they were paid, whether they were exposed to certain content, they were not naturally expected to see, like watching porn, cut bodies, and so on.

% I think approval is a different thing. It is up to the institution where the researchers are from, but I think on the very generic case we just want to make sure that the crowd workers were told in advance. For example, in the title of the task, it was clear what type of content they might find. So that would be one story.




==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> preamble.tex <==
\section{Preamble}

\textbf{Scope.} This paper aims to propose a datasheet for reporting crowdsourcing experiments. By crowdsourcing experiments, we mean studies that answer research questions/hypotheses using an experimental design (randomized or quasi-experimental) and crowd workers as participants (recruited from a crowdsourcing platform)\footnote{Human subjects should come from an online platform dedicated explicitly to crowdsourcing (paid or volunteering). Further details related to the scope can be found at \url{https://docs.google.com/document/d/1J-0ELGilVNfK_Y6rwX9JLNMupA_apo83FZLE76qz64A/edit?usp=sharing}}.
%
The motivation behind this work is that, currently, there are no standardized guidelines for reporting crowdsourcing projects, and crowdsourcing involves articulating many pieces that can certainly play a role in the results obtained (emphasizing the need for proper reporting).


\textbf{Progress so far.} We have built an initial taxonomy of relevant attributes characterizing crowdsourcing experiments. This taxonomy was derived from different sources 1) guidelines for experimental research, 2) guidelines for crowdsourcing experiments, 3) task design features in crowdsourcing platforms, and 4) papers reporting crowdsourcing experiments. 

We also collected papers by querying on Scopus and checking past HCOMP proceedings. We identified 175 relevant articles from the initial list of 994 documents that we obtained. These relevant studies report crowdsourcing experiments, based on the definition we introduced previously. Using a sample of the relevant papers, we plan to analyze and state of reporting according to the datasheet that we propose in this work.


\textbf{Validity of our work}. To validate our work, we seek to involve experts from the community to review our proposed taxonomy to update and improve it accordingly, growing it into a reporting tool.
%
Guided by our taxonomy, we also plan to rely on existing literature to distill how the different configuration of the parameters of crowdsourcing experiments could play a role in the results (e.g., different task interfaces, payments, instructions, demographics).

In our CSCW poster, we already identified what parameters tend to go underreported, so we are working on doing a complementary analysis, based on simulations from an existing crowdsourcing dataset, of how these underreported settings may flip or "dissolve" the results obtained from the controlled crowdsourcing experiments. Concretely, we are currently evaluating the sampling of workers based on demographics and time of the day, and how this could influence the results.
\gd{there seems to be an assumption that it would be good to report as much as possible. On the other hand, making MTurk output files available to the public may not be desirable as they contain worker IDs (see \url{https://blog.humancomputation.com/?p=5177}). Perhaps it could use useful to a para on the trade-offs between underreporting and overreporting.}
\jr{Regarding the sharing of output datasets, we'd make it clearer that by sharing results (e.g., raw judgments), we also ask for proper anonymization since, indeed, and thanks for sharing the link, workers are not anonymous. And yes, it would be great to discuss under- vs. over-reporting and address this with the datasheet.}

\textbf{Follow-up work}. In this paper, we scope the datasheet to crowdsourcing experiments. However, data collection (e.g., labeling for ML) is also a huge use case for crowdsourcing, and we aim to propose a taxonomy for reporting crowdsourced data collection. AAAI is a potential venue for this work.
